CodeT: Code Generation with Generated Tests

The task of generating code solutions for a given programming problem can benefit from the use of pre-trained language models such as Codex, which can produce multiple diverse samples. However, a major challenge for this task is to select the most appropriate solution from the multiple samples generated by the pre-trained language models. A natural way to evaluate the quality and correctness of a code solution is to run it against a set of test cases, but the manual creation of such test cases is often costly and time-consuming. In this paper, we propose a novel method, CodeT, that leverages the same pre-trained language models to automatically generate test cases for the code samples, thus reducing the human effort and increasing the coverage of the test scenarios. CodeT then executes the code samples using the generated test cases, and performs a dual execution agreement, which considers both the consistency of the outputs against the generated test cases and the agreement of the outputs with other code samples. We conduct comprehensive experiments on four benchmarks, HumanEval, MBPP, APPS and CodeContests, using five different pre-trained language models with varying sizes and capabilities. Our results show that CodeT can significantly improve the performance of code solution selection over previous methods, achieving remarkable and consistent gains across different models and benchmarks. For instance, CodeT improves the pass@1 metric on HumanEval to 65.8%, which represents an absolute improvement of 18.8% over the code-davinci-002 model, and an absolute improvement of more than 20% over the previous state-of-the-art results.

==> CodeT_ Code Generation with Generated Tests (arXiv V2 20221123)/0_abstract.tex <==
%With the recent development of pre-trained language models for code, code generation has attracted a great deal of attention. 
%Given a programming problem, pre-trained language models such as Codex have demonstrated the ability to generate multiple different code solutions via sampling. However, selecting a correct or best solution from those samples still remains a challenge. While an easy way to verify the correctness of a code solution is through executing test cases, producing high-quality test cases is prohibitively expensive. 
%In this paper, we explore the use of pre-trained language models to automatically generate test cases, calling our method \ours: \textsc{Code} generation with generated \textsc{T}ests. \ours executes the code solutions using the generated test cases, and then chooses the best solution based on a dual execution agreement with both the generated test cases and other generated solutions. We evaluate \ours on five different pre-trained models with both HumanEval and MBPP benchmarks. Extensive experimental results demonstrate \ours can achieve significant, consistent, and surprising improvements over previous methods. For example, 
%In this paper, we propose a simple yet effective approach, called \ours, which explores the use of pre-trained language models to automatically generate test cases, 
%unleashing the inherent power of pre-trained language models. Taking advantage of the generated test cases, we execute the code solutions and select the correct one base on execution agreement.
%Experimental results on the HumanEval and MBPP benchmarks demonstrate the superiority of \ours, for example, 
%\ours improves the pass@$1$ on HumanEval to $65.8\%$, an increase of absolute $18.8\%$ on the \davincitwo model, and an absolute $20$+$\%$ improvement over previous state-of-the-art results. 


%\textcolor{red}{
%The task of generating code solutions for a given programming problem can benefit from the use of pre-trained language models (PLMs) such as Codex, which can produce multiple diverse samples. However, a major challenge for this task is to select the most appropriate solution from the multiple samples generated by the PLMs. A natural way to evaluate the quality and correctness of a code solution is to run it against a set of test cases, but the manual creation of such test cases is often costly and time-consuming. 
%In this paper, we propose a novel method, \ours, that leverages the same PLMs to automatically generate test cases for the code samples, thus reducing the human effort and increasing the coverage of the test scenarios. \ours then executes the code samples using the generated test cases, and ranks them based on a dual execution agreement criterion, which considers both the consistency of the outputs against the generated test cases and the agreement of the outputs with other code samples. We conduct comprehensive experiments on two benchmarks, HumanEval and MBPP, using five different PLMs with varying sizes and capabilities. Our results show that \ours can significantly improve the performance of code solution selection over previous methods, achieving remarkable and consistent gains across different PLMs and benchmarks. For instance, 
%\ours improves the pass@$1$ metric on HumanEval to $65.8\%$, which represents an absolute improvement of $18.8\%$ over the \davincitwo model, and an absolute improvement of more than $20\%$ over the previous state-of-the-art results.}

The task of generating code solutions for a given programming problem can benefit from the use of pre-trained language models such as Codex, which can produce multiple diverse samples. However, a major challenge for this task is to select the most appropriate solution from the multiple samples generated by the pre-trained language models. A natural way to evaluate the quality and correctness of a code solution is to run it against a set of test cases, but the manual creation of such test cases is often costly and time-consuming. 
In this paper, we propose a novel method, \ours, that leverages the same pre-trained language models to automatically generate test cases for the code samples, thus reducing the human effort and increasing the coverage of the test scenarios. 
\ours then executes the code samples using the generated test cases and performs a dual execution agreement, which considers both the consistency of the outputs against the generated test cases and the agreement of the outputs with other code samples. 
We conduct comprehensive experiments on four benchmarks, HumanEval, MBPP, APPS, and CodeContests, using five different pre-trained language models with varying sizes and capabilities. Our results show that \ours can significantly improve the performance of code solution selection over previous methods, achieving remarkable and consistent gains across different models and benchmarks. For instance, 
\ours improves the pass@$1$ metric on HumanEval to $65.8\%$, which represents an absolute improvement of $18.8\%$ over the \davincitwo model, and an absolute improvement of more than $20\%$ over the previous state-of-the-art results.

==> CodeT_ Code Generation with Generated Tests (arXiv V2 20221123)/1_introduction.tex <==
\section{Introduction}\label{sec:intro}

%Code generation has been a long-standing topic in the research community, as we have a dream that code can learn to code itself. 
%Thanks to the recent advances in pre-training techniques, many large language models have been pre-trained for code generation, e.g., Codex~\citep{chen2021evaluating},  AlphaCode~\citep{li2022competition}, \incoder~\citep{dfried2022incoder}, \codegen~\citep{Nijkamp2022ACP} and PolyCoder~\cite{xu2022PolyCoder}, as well as bringing code generation into real-world applications such as Copilot\footnote{\url{https://github.com/features/copilot}}. While these advanced pre-trained models are able to generate many different solutions for a programming problem via sampling, it remains a challenge to select a single correct solution from multiple generated candidates. Taking the HumanEval benchmark~\citep{chen2021evaluating} as an example, Codex has a pass$@100$ (pass if one or more among $100$ generated solutions for a given problem can pass the corresponding test cases) of $77.4\%$, but a pass$@1$ (correct rate of a single  solution) of only $33.5\%$\footnote{Results on the HumanEval benchmark with \cushman. More results can be found in Section \ref{sec:mainres}.}. This huge gap makes it imperative to explore how to pick the correct or best  solution from multiple candidates.
%The huge gap made us think about the question: 
%Can the pre-trained models help themselves to select the correct code solution?
%how can we select the correct code solution from multiple candidates in a simple way?

%\textcolor{red}{
%Despite the remarkable progress in pre-training techniques for code generation, selecting a single correct solution from multiple candidates generated by large language models remains a hard problem. For instance, Codex~\citep{chen2021evaluating}, a state-of-the-art pre-trained model for code generation, can produce up to $100$ different solutions for a given programming problem, but only one third of them can pass the test cases on the HumanEval benchmark~\citep{chen2021evaluating}\footnote{We report the results on the HumanEval benchmark with \cushman, the largest publicly available Codex model. More results with different models and benchmarks can be found in Section \ref{sec:mainres}.}. This huge gap limits the practical usefulness of code generation models and motivates us to explore how to pick the correct or best  solution from multiple candidates.
%}

Despite the remarkable progress in pre-training techniques for code generation, selecting a single correct solution from multiple candidates generated by large language models remains a hard problem. 
For instance, Codex~\citep{chen2021evaluating}, a state-of-the-art pre-trained language model for code generation, can achieve a pass$@100$ (pass if one or more among $100$ generated solutions for a given problem can pass the corresponding test cases) of $77.4\%$, but a pass$@1$ (correct rate of a single  solution) of only $33.5\%$ on the HumanEval benchmark~\citep{chen2021evaluating}\footnote{We report the results on the HumanEval benchmark with the Codex model \cushman. More results with different models and benchmarks can be found in Section \ref{sec:mainres} and \ref{sec:exp_apps_codecontests}}. 
This huge gap limits the practical usefulness of code generation models and motivates us to explore how to pick the correct or best solution from multiple candidates.

%A simple way to verify the correctness of a  solution is to execute it and then check if it passes all corresponding test cases. Such an execution-guided approach has been extensively applied to many code-related tasks, such as code generation~\citep{chen2021evaluating,li2022competition,shi2022natural}, code translation~\citep{roziere2021leveraging}, and program synthesis~\citep{chen2018execution,ellis2019write}. 
%The challenge, however, is that preparing a sufficient number of high-quality test cases to cover all the corner cases is prohibitively expensive and inefficient. 
%In real-world applications like Copilot, %it is discouraging to ask users to provide test cases when they are using a code generation tool. 
%it is troublesome if users are required to provide test cases when they are using a code generation tool. 
%To address these challenges, we explore approaches to automatically produce test cases for arbitrary programming problems and then use them to quickly verify any solution.

%\textcolor{red}{
%A straightforward way to verify the correctness of a  solution is to execute it and compare its output with the expected output for each test case. This execution-guided approach has been widely adopted in various code-related tasks, such as code generation~\citep{chen2021evaluating,li2022competition,shi2022natural}, code translation~\citep{roziere2021leveraging}, and program synthesis~\citep{chen2018execution,ellis2019write}. 
%However, this approach relies heavily on the quality and quantity of the test cases, which are often costly and time-consuming to create and maintain. Moreover, in real-world applications like Copilot, a code generation tool that assists developers in writing code, it is not realistic to expect users to provide test cases for every problem they want to solve. Therefore, we propose to automatically generate test cases for arbitrary programming problems and use them to quickly verify any solution.
%}

A straightforward way to verify the correctness of a  solution is to execute it and check if it passes all corresponding test cases. This execution-guided approach has been widely adopted in various code-related tasks, such as code generation~\citep{chen2021evaluating,li2022competition,shi2022natural}, code translation~\citep{roziere2021leveraging}, and program synthesis~\citep{chen2018execution,ellis2019write}. 
However, this approach relies heavily on the quality and quantity of test cases, which are often costly and time-consuming to create and maintain. Moreover, in real-world applications like Copilot\footnote{\url{https://github.com/features/copilot}}, a code generation tool that assists developers in writing code, it is unrealistic to expect users to provide test cases for every problem they want to solve. Therefore, we propose to automatically generate test cases for arbitrary programming problems and use them to quickly verify any solution.

%A few attempts have tried to train a ranker~\citep{cobbe2021training,shen2021generate,inala2022fault}. (need training data and extra module)

%When it comes to choosing among multiple code solutions, the most straightforward way is to work with test cases to obtain execution results. \cite{shi2022natural} executed code solutions with a number of test case inputs, and then selected a solution whose output had the maximal agreement with the others. Though effective, it requires additional test case inputs. 
%In this work, we would like to make it more elegant by unleashing the inherent power of pre-trained models to help themselves. The main idea is quite simple: bootstrap code generation with synthesized test cases using a single model. It is based on two hypotheses: (1) People think differently, while different thoughts often lead to the same correct answer, and the same goes for pre-trained models. (2) Pre-trained models can generate code for a programming problem, as well as the corresponding test cases. 

%\bei{to be modified:} Although pre-trained models such as Codex have been used to generate code solutions, we start by designing an elaborate instruction as prompt, asking the same language model to automatically generate large amounts of test cases for each programming problem, as illustrated in  Figure \ref{fig:illustration}. 
%Second, we execute each of the generated solutions on the generated test cases to associate each solution with all the test cases it can pass.
%Second, we execute the generated test cases on each of the generated solution to record to associate each solution with all the test cases it can pass. 
%Third, we apply a dual execution agreement on both the solutions and the test cases. We believe a solution could get support from both the test cases and the other solutions. The more test cases a solution can pass, the better the solution is. Meanwhile, if there is another test-driven sibling solution that could pass the exact same test cases as the current solution, it is likely that the two solutions have the same functionality, although with different implementations. We regard the sibling solutions as  supporting each other where a larger number of sibling solutions can directly contribute to the correctness of a solution. Finally, we calculate a ranking score based on this dual execution agreement and produce the best solution. We call our method \ours: \textsc{Code} generation with generated \textsc{T}est-driven dual execution agreement. 

%\textcolor{red}{
%Our method, which we call \ours: \textsc{Code} generation with generated \textsc{T}est-driven dual execution agreement, consists of three main steps, as illustrated in  Figure \ref{fig:illustration}. First, we leverage the same pre-trained model that generates code solutions, such as Codex, to generate a large number of test cases for each programming problem, by providing an elaborate instruction as prompt. Second, we execute each of the generated solutions on the generated test cases and record the number of test cases that each solution can pass. Third, we rank the solutions based on a dual execution agreement, which considers both the test cases and the other solutions as evidence for the correctness of a solution. Intuitively, a solution that can pass more test cases is more likely to be correct, and a solution that has more sibling solutions, i.e., solutions that can pass the same test cases, is more likely to have the same functionality as the problem specification, even if they have different implementations. We compute a ranking score for each solution based on this dual execution agreement and select the best solution. }

%In this paper, we propose \ours: \textsc{Code} generation with generated \textsc{T}est-driven dual execution agreement, as illustrated in  Figure \ref{fig:illustration}. First, we leverage the same pre-trained language model that generates code solutions, such as Codex, to generate a large number of test cases for each programming problem, by providing an elaborate instruction as prompt. 
%Then, inspired by the idea of classical RANSAC algorithm \citep{fischler1981random}, we perform a dual execution agreement between code solutions and test cases. Specifically, we execute each of the generated solutions on the generated test cases, and design an iterative manner to obtain multiple consensus sets. Each consensus set consists of multiple pairs of code solutions and test cases. Code solutions in the same consensus set can pass the same test cases, showing that they have the same functionality, even though they may vary in implementation. 
%Intuitively, a solution that can pass more test cases is more likely to be correct, and a solution with more siblings, i.e., solutions in the same consensus set, is more likely to have the correct functionality as the problem specification. 
%Therefore, we compute the ranking score for each consensus set based on both the test cases and code solutions in it, and select the best solution from the consensus set with the highest score. 


In this paper, we propose \ours: \textsc{Code} generation with generated \textsc{T}est-driven dual execution agreement, as illustrated in  Figure \ref{fig:illustration}. First, we leverage the same pre-trained language model that generates code solutions, such as Codex, to generate a large number of test cases for each programming problem by providing an elaborate instruction as prompt. 
Next, we use a dual execution agreement approach inspired by the classical RANSAC algorithm \citep{fischler1981random}. We execute each generated code solution on each generated test case, and iteratively find multiple groups of code solution and test case pairs. Each group, or consensus set, has solutions that pass the same test cases, indicating that they have the same functionality, even if they are different in implementation. 
We expect that a solution that passes more test cases is more correct, and that a solution that has more similar solutions, i.e., solutions in the same consensus set, is more consistent with the problem specification. 
So, we rank each consensus set by both the number of test cases and solutions in it, and choose the best solution from the highest-ranked consensus set. 

%Although \ours is simple and efficient,  without any need of either labelled data or additional rankers, its performance is surprisingly exceptional. We evaluate \ours on five different pre-trained models: three OpenAI Codex models~\citep{chen2021evaluating}, \incoder~\citep{fried2022incoder}, and \codegen~\citep{Nijkamp2022ACP}, as well as four established benchmarks: HumanEval~\citep{chen2021evaluating},  MBPP~\citep{austin2021program}, APPS~\cite{hendrycks2021measuring}, and CodeContests~\cite{li2022competition}. Extensive experimental results show \ours can effectively select the correct solution, boosting the pass$@1$ score significantly: HumanEval ($33.5\% \to 44.5\%$ with \cushman and $47.0\% \to 65.8\%$ with \davincitwo), MBPP ($45.9\% \to 55.4\%$ with \cushman and $58.1\% \to 67.7\%$ with \davincitwo), APPS ($8.9\% \to 12.2\%$ with \davincitwo), and CodeContests ($0.7\% \to 2.1\%$ with \davincitwo). %Especially, via combining \davincitwo and \ours, it outperforms previous state-of-the-art methods by a large margin on both benchmarks (HumanEval: $42.7\%$ \citep{inala2022fault} $\to 65.8\%$ and MBPP: $xxx \to 67.7\%$).
%Furthermore, combining \davincitwo and \ours  outperforms previous state-of-the-art methods by a large margin, e.g.,  HumanEval: $42.7\%$ \citep{inala2022fault} $\to 65.8\%$.
%We will make most of our code and data publicly available. 
%Our work will be publicly available at \url{https://github.com/microsoft/CodeT}.
%Our work will be publicly available upon acceptance.

%\textcolor{red}{
%Our method is simple and efficient, as it does not require any labelled data or additional rankers, but it achieves surprisingly exceptional performance. We evaluate our method on five different pre-trained models for code generation: three OpenAI Codex models~\citep{chen2021evaluating}, \incoder~\citep{fried2022incoder}, and \codegen~\citep{Nijkamp2022ACP}, as well as four established benchmarks for code generation: HumanEval~\citep{chen2021evaluating},  MBPP~\citep{austin2021program}, APPS~\cite{hendrycks2021measuring}, and CodeContests~\cite{li2022competition}. The experimental results show that our method can effectively select the correct solution from multiple candidates, improving the pass$@1$ score significantly on all benchmarks: HumanEval ($33.5\% \to 44.5\%$ with \cushman and $47.0\% \to 65.8\%$ with \davincitwo), MBPP ($45.9\% \to 55.4\%$ with \cushman and $58.1\% \to 67.7\%$ with \davincitwo), APPS ($8.9\% \to 12.2\%$ with \davincitwo), and CodeContests ($0.7\% \to 2.1\%$ with \davincitwo). %Especially, via combining \davincitwo and \ours, it outperforms previous state-of-the-art methods by a large margin on both benchmarks (HumanEval: $42.7\%$ \citep{inala2022fault} $\to 65.8\%$ and MBPP: $xxx \to 67.7\%$).
%Moreover, when we combine \davincitwo, the most powerful pre-trained model, and \ours, we outperform previous state-of-the-art methods by a large margin, e.g.,  HumanEval: $42.7\%$ \citep{inala2022fault} $\to 65.8\%$. We also conduct extensive ablation studies to validate the effectiveness of each component in our method. Our code and data are publicly available\footnote{\url{https://github.com/ccasclab/CodeTTA}}.}

Our method is simple and efficient, as it does not require any labelled data or additional rankers, but it achieves surprisingly exceptional performance. We evaluate our method on five different pre-trained language models for code generation: three OpenAI Codex models~\citep{chen2021evaluating}, \incoder~\citep{fried2022incoder}, and \codegen~\citep{Nijkamp2022ACP}, as well as four established benchmarks for code generation: HumanEval~\citep{chen2021evaluating},  MBPP~\citep{austin2021program}, APPS~\citep{hendrycks2021measuring}, and CodeContests~\citep{li2022competition}. The experimental results show that our method can effectively select the correct solution from multiple candidates, improving the pass@$1$ score significantly on all benchmarks in the zero-shot setting. For instance, \ours achieves improvements using \davincitwo: HumanEval ($47.0\% \to 65.8\%$), MBPP ($58.1\% \to 67.7\%$), APPS \textsc{Introductory} ($27.2\% \to 34.6\%$), and CodeContests ($0.7\% \to 2.1\%$). %Especially, via combining \davincitwo and \ours, it outperforms previous state-of-the-art methods by a large margin on both benchmarks (HumanEval: $42.7\%$ \citep{inala2022fault} $\to 65.8\%$ and MBPP: $xxx \to 67.7\%$).
Moreover, when we combine \davincitwo, the most powerful pre-trained model, and \ours, we outperform previous state-of-the-art methods by a large margin, e.g.,  HumanEval: $42.7\%$ \citep{inala2022fault} $\to 65.8\%$. 
We also conduct a thorough analysis to provide more insights. Our work is publicly available at \url{https://github.com/microsoft/CodeT}.

%In this paper, we propose \ours to boost {\bf{\textsc{Code}}} generation with synthesized {\bf\textsc{T}}est-driven Execution Agreement. We make test case generation more elegant by unleashing the inherent power of the pre-trained language models. As the illustration shown in Figure \ref{fig:illustration}, we use the pre-trained language model to generate code solutions for each programming problem, while test cases are automatically generated using the same model by designing a special instruction. Then the code solutions are executed on the test cases, and we select the final code solution based on the idea of execution agreement:  
%the code solution that is agreed upon by the most others is the most likely to be correct. 
%\ours is simple without introducing any extra information and module. We conduct experiments with analysis on two code generation benchmarks. Experimental results show \ours can effectively select the correct code solution, boosting the pass$@1$ score significantly: HumanEval ($33.5\% \to 44.5\%$ with \cushman and $47.0\% \to 65.8\%$ with \davincitwo), and MBPP ($45.9\% \to 55.4\%$ with \cushman and $58.1\% \to 67.7\%$ with \davincitwo).




%Based on the hypotheses, we propose our method called \ours. The illustration is shown in Figure \ref{fig:illustration}. For a specific programming problem, we employ Codex and perform zero-shot code generation to obtain a set of \emph{code solutions}. At the same time, a special designed instruction is added to perform zero-shot test case generation, resulting in a set of \emph{test cases}. Then, leveraging execution results, a dual-agreement operation is performed between code solutions and test cases, where they score each other. The code solution with highest agreement score is selected as the final one. 
%The method is simple without introducing any extra information and module. We conduct experiments with analysis on XX benchmarks. Experimental results show \ours can effectively select the correct code solution, boosting the pass$@1$ score significantly: HumanEval ($X\% \to X\%$), MBPP ($X\% \to X\%$) XXX.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{illustration-v3.pdf}
    \caption{The illustration of \ours. Both the code solutions and the test cases are generated by the pre-trained language model. The best code solution is then selected by a dual execution agreement.}
    \label{fig:illustration}
\end{figure}

==> CodeT_ Code Generation with Generated Tests (arXiv V2 20221123)/2_method.tex <==
\section{Methodology} \label{sec:method}


%If a code solution is agreed by more test cases and more code solutions, then it is more likely to be correct.

The task of code generation is to solve a programming problem: generate \emph{code solution} $x$ based on \emph{context} $c$. As shown in Figure \ref{fig:prelimilary}, context $c$ contains natural language problem description in the form of code comment, and a code snippet that includes statements such as imports and the function header. A code solution is a code snippet that solves the programming problem described in the context. Generally, we sample a set of code solutions, denoted as $\mathbf{X}=\{x_1,x_2,{\cdots},x_N\}$, based on the context $c$ using a pre-trained language model $\mathcal{M}$, which can be formulated as $\mathbf{X}=\mathcal{M}(c)$.
Our goal is to select the best code solution $\hat{x}$ from the set of generated code solutions $\mathbf{X}$, where $\hat{x}$ is the most likely solution to correctly solve the given programming problem. To this end, we propose \ours in the hope of unleashing the inherent power of the pre-trained language model $\mathcal{M}$. Specifically, we use $\mathcal{M}$ to generate test cases for the programming problem (Section \ref{sec:testcase}), and then select the best code solution $\hat{x}$ based on a dual execution agreement (Section \ref{sec:agree}).

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{preliminary-v2.pdf}
    \caption{Code generation and test case generation: an example from the HumanEval benchmark. Example input-output cases are removed from the context.}% Background colors: light grey for context $c$, grey for instruction $p$, yellow for code solutions $\mathbf{x}$ and blue for test cases $\mathbf{y}$.}
    \label{fig:prelimilary}
\end{figure}




\subsection{Test Case Generation}
\label{sec:testcase}
%We leverage the pre-trained language model $\mathcal{M}$ to generate both code solutions and test cases. When generating test cases, to tell the model that we want to generate test cases rather than code solutions, we add an \emph{instruction} $p$ as a prompt following the context $c$. As shown in Figure \ref{fig:prelimilary}, we construct instruction $p$ using the following parts: a ``${\rm{pass}}$" statement as a placeholder of the function body, a comment ``check the correctness of [entry point]" to clarify the intention of generating test cases, and an ``${\rm{assert}}$" to kick off the test case generation. The process of test case generation can be formulated as $\mathbf{y}=\mathcal{M}({\rm{concat}}(c,p))$, where $\mathbf{y}=\{y_1,y_2,{\cdots},y_M\}$ denotes a set of test cases and ${\rm{concat}}$ is the concatenation operation. It is worth noting that we remove all example input-output cases from the context $c$ to avoid exposing real test cases.


%\textcolor{red}{
%Besides generating code solutions, we also need to generate test cases to evaluate the correctness of the code solutions. A test case is a pair of input and expected output for the function defined in the context. For example, in Figure \ref{fig:prelimilary}, a test case for the programming problem of checking whether there exist close elements in a list less than a threshold. To generate test cases, we use the same pre-trained language model $\mathcal{M}$ that we use for generating code solutions, but we add an \emph{instruction} $p$ to the context $c$ as a prompt to indicate that we want test cases instead of code solutions. The instruction $p$ consists of three parts: (1) a ``${\rm{pass}}$" statement as a placeholder of the function body, which signals that we do not need to generate code for the function, (2) a comment ``check the correctness of [entry point]" to clarify the intention of generating test cases, where [entry point] is the name of the function, and (3) an ``${\rm{assert}}$" statement to start the test case generation, which specifies the format of the test cases as input-output pairs. For instance, Figure \ref{fig:prelimilary}, provides an example of the instruction $p$.
%}

%\textcolor{red}{
%We then feed the concatenated context and instruction, ${\rm{concat}}(c,p)$, to the language model $\mathcal{M}$, and sample a set of test cases, denoted as $\mathbf{y}=\{y_1,y_2,{\cdots},y_M\}$, from the model output. The language model will try to complete the instruction by generating plausible input-output pairs for the function. 
%Note that we remove all example input-output cases from the context $c$ before generating test cases, to avoid exposing real test cases to the language model and to increase the diversity and difficulty of the generated test cases. The process of test case generation can be formulated as $\mathbf{y}=\mathcal{M}({\rm{concat}}(c,p))$.}

Besides generating code solutions, we also need to generate test cases to evaluate the correctness of the code solutions. A test case is a pair of input and expected output for the function defined in the context. For example, in Figure \ref{fig:prelimilary}, a test case for the programming problem of checking whether there exist close elements in a list less than a threshold. To generate test cases, we use the same pre-trained language model $\mathcal{M}$ that we use for generating code solutions, but we add an \emph{instruction} $p$ to the context $c$ as a prompt to indicate that we want test cases instead of code solutions. As shown in Figure \ref{fig:prelimilary}, the instruction $p$ consists of three parts: (1) a ``${\rm{pass}}$" statement as a placeholder of the function body, which signals that we do not need to generate code for the function, (2) a comment ``check the correctness of [entry point]" to clarify the intention of generating test cases, where ``[entry point]" is the name of the function, and (3) an ``${\rm{assert}}$" statement to start the test case generation, which specifies the format of the test cases as input-output pairs.

We then feed the concatenated context and instruction, ${\rm{concat}}(c,p)$, to the language model $\mathcal{M}$, and sample a set of test cases, denoted as $\mathbf{Y}=\{y_1,y_2,{\cdots},y_M\}$, from the model output. The process of test case generation can be formulated as $\mathbf{Y}=\mathcal{M}({\rm{concat}}(c,p))$. The language model will try to complete the instruction by generating plausible input-output pairs for the function. 
Note that we remove all example input-output cases from the context $c$ before generating code solutions and test cases, to avoid exposing real test cases to the language model and to increase the diversity and difficulty of the generated test cases. %The process of test case generation can be formulated as $\mathbf{y}=\mathcal{M}({\rm{concat}}(c,p))$.

\iffalse
\subsection{Dual Execution Agreement (original version)}
\label{sec:agree}
%In this subsection, we try to answer the question: given the code solutions $\mathbf{x}$ and the test cases $\mathbf{y}$, how do we select the solution $\hat{x}$ that is most likely correct?
In this subsection, we try to answer the question: given the code solutions $\mathbf{X}=\{x_1,x_2,{\cdots},x_K\}$ and the test cases $\mathbf{Y}=\{y_1,y_2,{\cdots},y_M\}$, how do we select the solution $\hat{x}$ that is most likely correct?

First, we execute each of the generated code solutions on the generated test cases. Then, the most straightforward way is to score each code solution by the number of test cases it can pass. However, we found this naive method is not good enough\footnote{Results can be found in Section \ref{sec:mainres}.}. A simple example is shown in Figure \ref{fig:agree}. There are three code solutions and five test cases for the programming problem ``return the square of a number''. The highest scoring code solution is $x_3$, which passes four test cases. $x_3$, however, is obviously not the correct solution, since it returns the double of a number, not its square. As observed, although $x_1$ and $x_2$ are two different solutions, they are both correct with the same functionality of returning the square of a number. Hence, it is reasonable for them to group together. By adding up the scores of $x_1$ and $x_2$, they will be selected based on a combined score of $6$.  

\modify{
We hold two assumptions that align with the idea of the classical RANSAC algorithm \citep{fischler1981random}: (1) all the code solutions and test cases are sampled independently and randomly, and (2) the probability density of correct samples is greater then that of noisy samples. Hence, there are enough correct samples to agree on a correct functionality, and noisy samples will not agree consistently on any single functionality. Based on the assumptions, we propose our approach \ours to perform what we call dual execution agreement.
}
%Based on this idea, we propose our approach \ours to perform what we call dual execution agreement. 
Formally, for each code solution $x\in \mathbf{x}$, we execute it with all test cases in $\mathbf{y}$. If two code solutions can pass a same set of test cases, 
then they are sibling solutions with the same functionality; thus, we can put them into the same cluster. In this way, all code solutions in $\mathbf{x}$ can be divided into several clusters, denoted as $\mathbf{x}=\{\mathbf{x}_1,\mathbf{x}_2,{\cdots},\mathbf{x}_N\}$. Let $W=\{w_{ij}\}$ be an $N\times M$ matrix to represent the execution results, where $N$ is the number of code solution clusters and $M$ is the number of test cases. If code solutions in cluster $\mathbf{x}_i$ can pass the test case $y_j$, then $w_{ij}=1$; otherwise, $w_{ij}=0$. 
\modify{Recalling the assumptions stated before, }the basic idea of the dual execution agreement is that
a good code solution should be agreed upon by both the test cases and the other solutions: (1) The more test cases it can pass, the better the solution is. (2) A larger number of sibling solutions can directly contribute to the correctness of the solution. 
%To keep the notation simple, we also use $\mathbf{x}_i$ and $y_j$ to denote their scores.
Hence, we define the score of each cluster $\mathbf{x}_i$ to be:
\begin{equation}\label{eq:agree}
%f(\mathbf{x}_i) = N_i^{\frac{1}{2}} \sum_{j=1}^M w_{ij} \cdot g_0(y_j),
%f(\mathbf{x}_i) = r_i \sum_{j=1}^M w_{ij}  g_0(y_j),
f(\mathbf{x}_i) = |\mathbf{x}_i| \sum_{j=1}^M w_{ij},
\end{equation}
%where $g_0(y_j)=\frac{1}{M}$ denotes the initial normalized score of test case $y_j$ and $r_i$ 
where $|\mathbf{x}_i|$ is the code solution number in cluster $\mathbf{x}_i$.
%$r_i$ is the square root of the code solution number in the cluster $\mathbf{x}_i$. We use the square root to reduce the impact caused by code solutions due to the intuition that the number of code solutions is less important than the number of test cases. For example, there may be one code solution that can pass five test cases, whereas another five code solutions may pass only one test case. We intuitively consider that the former may be more likely correct. 
Finally, we get the best code solution $\hat{x}$ by selecting any code solution from the highest scoring cluster. In addition, if we want to obtain $k$ code solutions, we can select one code solution from each of the top $k$ highest scoring clusters.
\fi

%\subsection{\oursiter}
%In \ours, each test case contributes equally to the score of the code solution. So the question arises: do different test cases have different levels of importance? Intuitively, if a test case can be passed by more code solutions, the more likely the test case is to be correct. 
%To this end, we further propose \oursiter to consider the importance of test cases in an iterative manner. Inspired by the work for bipartite graph ranking~\citep{kleinberg1999authoritative,he2016birank,yang2020birank}, the scores of $\mathbf{x}_i$ and $y_j$ can be calculated as:
%\begin{equation}\label{eq:iter}
%\begin{aligned}
%f(\mathbf{x}_i) =& \alpha r_i \sum_{j=1}^M w_{ij} g(y_j)+ (1-\alpha) f_0(\mathbf{x}_i),\\
%g(y_j) =& \beta \sum_{i=1}^N w_{ij} f(\mathbf{x}_i) + (1-\beta) g_0(y_j),
%\end{aligned}
%\end{equation}
%where $f_0(\mathbf{x}_i)=r_i/\sum_{n=1}^N r_n$ is the initial normalized score of $\mathbf{x}_i$, and $\alpha$ and $\beta$ are hyper-parameters to be set between $[0,1]$ to account for the importance of the initial scores. The scores of $\mathbf{x}_i$ and $y_j$ are calculated iteratively using Equation \ref{eq:iter}. For convergence, the scores of all code solution clusters are normalized after each iteration; the same applies to the test cases as well.

%\subsection{Dual Execution Agreement (RANSAC version)}
% In this subsection, we try to answer the question: given the code solutions $\mathbf{x}=\{x_1,x_2,{\cdots},x_K\}$ and the test cases $\mathbf{y}=\{y_1,y_2,{\cdots},y_M\}$, how do we select the solution $\hat{x}$ that is most likely correct?
 
 %For a given natural language specification $c$, we denote all code snippets that can correctly implement the intent of $c$ as a set $V_x(c)$, which is a subset of all code snippets $\Omega_x$ that can be generated by the model.
 %All incorrect code snippets can be denoted as $NV_x=\Omega_x(c) - $
 %In this paper, we take an assumption that the errors in the generated code snippets by the model are randomly distributed over the set 
 %Similarly, we denote all valid test cases as $V_y$ and it is a subset of all possible test cases $\Omega_y(c)$.
 %Then, the code snippet (or test case) generation can be considered as sampling a code snippet $x$ (or test case $y$) from the set $\Omega_x(c)$ (or $\Omega_y(c)$) based on a given context $c$. 
 
\subsection{Dual Execution Agreement}
\label{sec:agree}
%In this subsection, we try to answer the question: given the code solutions $\mathbf{x}=\{x_1,x_2,{\cdots},x_K\}$ and the test cases $\mathbf{y}=\{y_1,y_2,{\cdots},y_M\}$, how do we select the solution $\hat{x}$ that is most likely correct?

%\textcolor{red}{In this subsection, we explain how we select the best code solution $\hat{x}$ from the set of generated code solutions $\mathbf{x}=\{x_1,x_2,{\cdots},x_K\}$, using the set of generated test cases $\mathbf{y}=\{y_1,y_2,{\cdots},y_M\}$ as a criterion. }





%Both code solutions and test cases are sampled from the pre-trained language model $\mathcal{M}$ given a certain programming problem. 
%Each code solution $x\in\mathbf{x}$ can be executed on a test case $y\in\mathbf{y}$, making a pair $(x, y)$. 
%It is known that both a code solution and a test case can be a description of code functionality to some extent.
%Some of the $(x, y)$ pairs describe the correct functionality for the programming problem, and we call these pairs \emph{inliers}. Meanwhile, those pairs that fail to describe the correct functionality are called \emph{outliers}. 
%Taking Figure \ref{fig:agree} as an example, there are three code solutions and five test cases for the programming problem ``return the square of a number''. $(x_1,y_1)$ and $(x_2,y_2)$ are two of the inliers, where $x_1$ and $x_2$ are two different solutions with the same correct functionality of returning the square of a number. $(x_1,y_4)$ and $(x_3,y_2)$ are two of the outliers, because $y_4$ fails to describe the square of a number ($x_1$ cannot pass $y_4$) and $x_3$ describes the double of a number.
%For a reasonable good model, it is reasonable to assume that: (1) all samples (inliers and outliers) are drawn independently and randomly from the model, and (2) the probability density of inliers is greater than that of outliers. Hence, there are enough inliers to agree on a correct functionality, and  outliers will not agree consistently on any single functionality. These assumptions align with the idea of the classical RANSAC algorithm \citep{fischler1981random}, based on which we propose our approach \ours to perform what we call dual execution agreement. It is an iterative method, which we summarize as follows:


%\textcolor{red}{
%The idea is to find the code solution that can pass the most test cases, and that agrees with other code solutions that can pass the same test cases. We call this idea dual execution agreement, because it requires both the code solution and the test case to execute successfully and consistently. We base our idea on the assumptions that: (1) the code solutions and the test cases are independently and randomly sampled from the pre-trained language model $\mathcal{M}$ given a certain programming problem, and (2) the probability of sampling a correct code solution or a valid test case is higher than sampling an incorrect or invalid one. These assumptions imply that there are more code solutions and test cases that describe the correct functionality for the programming problem than those that do not, and that the correct ones will agree with each other more often than the incorrect ones. These assumptions are similar to those of the classical RANSAC algorithm \citep{fischler1981random}, which is a robust method for finding consensus among noisy data. Inspired by RANSAC, we propose our approach \ours to perform dual execution agreement. It is an iterative method, which we describe as follows:}

In this subsection, we explain how we select the best code solution $\hat{x}$ from the set of generated code solutions $\mathbf{X}=\{x_1,x_2,{\cdots},x_N\}$, using the set of generated test cases $\mathbf{Y}=\{y_1,y_2,{\cdots},y_M\}$ as a criterion.
%If a code solution $x$ can execute and pass a test case $y$, we call the pair $(x,y)$ a consistent pair.
We can execute a code solution $x$ on a test case $y$, which means running the function defined by $x$ on the input part of $y$ and comparing the output with the output part of $y$. If the code solution $x$ can be executed without errors and the output matches the expected output, then we say the code solution $x$ can pass the test case $y$. 
%A code solution $x$ can be executed on a test case $y$, forming a pair $(x,y)$. 
Furthermore, we say there is a functionality agreement between two code solutions $x_i$ and $x_j$ if they can pass the same set of test cases in $\mathbf{Y}$. 
%The idea is to find the code solution that can pass the most test cases, and that agrees with other . 
Our approach is based on the following assumptions: 
(1) the code solutions and the test cases are independently and randomly sampled from the pre-trained language model $\mathcal{M}$ given a certain programming problem, and 
(2) incorrect code solutions are often diverse, and the probability of having a functionality agreement between two incorrect code solutions by chance is very low.
%and it much lower than the probability of correct code solutions (or test cases) agreeing with each other is higher, while the  not agree consistently on any single functionality. 
These assumptions are similar to those of the classical RANSAC algorithm \citep{fischler1981random}, which is a robust method for finding consensus among noisy data.
Inspired by RANSAC, we propose our approach \ours to perform dual execution agreement, which is an iterative approach as follows: 
%We call this idea dual execution agreement, because it tests the functionality agreement among code solutions. 
%the probability of sampling a code solution (or test case) with the correct functionality is higer than sampling one with a specific incorrect functionality, meaning that the correct code solutions and test cases will agree with each other more often, while the incorrect ones are diverse and will not agree consistently on any single functionality. 
%It is an iterative method, which we describe as follows:


%\begin{itemize}
%    \item A pair $(x, y)$ is randomly selected from $\mathcal{D}=\{(x, y)|x\in\mathbf{x}, y\in\mathbf{y}\}$. If the code solution $x$ can be executed and pass the test case $y$, then $(x, y)$ is a hypothetical inlier (it is a hypotheses because we do not know whether it is a real inlier or not at current stage.); otherwise, it is an outlier. Figure \ref{fig:agree} shows a simple example of the programming problem ``return the square of a number''. $(x_1,y_1)$ and $(x_3,y_2)$ are two of the hypothetical inliers, while $(x_1,y_4)$ and $(x_3,y_1)$ are two of the outliers.
%    \item If $(x, y)$ is a hypothetical inlier, it can describe a hypothetical functionality. We propose to collect all pairs from $\mathcal{D}$ that fit this functionality, forming a set $\mathcal{S}$ called \emph{consensus set}. Specially, let $\mathcal{S}_y$ denote all test cases that $x$ can pass. We then find all code solutions that exactly can pass the test cases in $\mathcal{S}_y$, denoted as $\mathcal{S}_x$. Finally, the consensus set can be denoted as $\mathcal{S}=\{(x, y)|x\in\mathcal{S}_x, y\in\mathcal{S}_y\}$. For example in Figure \ref{fig:agree}, we can get $\mathcal{S}_x=\{x_1,x_2\}, \mathcal{S}_y=\{y_1,y_2,y_3\}$ from the hypothetical inlier $(x_1,y_1)$ (shown in green box), and $\mathcal{S}_x=\{x_3\}, \mathcal{S}_y=\{y_2,y_3,y_4,y_5\}$ from  $(x_3,y_2)$ (shown in purple box).
%    \item The consensus set can be scored as $f(\mathcal{S}) = |\mathcal{S}_x||\mathcal{S}_y|$, where $|\mathcal{S}_x|$ is the code solution number in $\mathcal{S}_x$ and $|\mathcal{S}_y|$ is the test case number in $\mathcal{S}_y$.
%    It equals to the number of pairs in the consensus set. Similar to that in RANSAC, the more pairs that fit the hypothetical functionality, the more likely this functionality will be correct, in line with our assumptions stated before. Following the example in Figure \ref{fig:agree}, the consensus set scores are $6$ and $4$ for the hypothetical inliers $(x_1,y_1)$ and $(x_3,y_2)$, respectively.
%\end{itemize}

%\textcolor{red}{
%\begin{itemize}
%    \item We randomly select a pair $(x, y)$ from the set of all possible pairs $\mathcal{D}=\{(x, y)|x\in\mathbf{x}, y\in\mathbf{y}\}$. We then try to execute the code solution $x$ on the test case $y$, which means to run the function defined by $x$ on the input part of $y$ and compare the output with the output part of $y$. If the code solution $x$ can be executed without errors and the output matches the expected output, then we say that the pair $(x, y)$ is a \emph{hypothetical inlier}, because it hypothetically describes the correct functionality for the programming problem. Otherwise, we say that the pair $(x, y)$ is an \emph{outlier}, because it fails to describe the correct functionality. Figure \ref{fig:agree} shows a simple example of the programming problem ``return the square of a number''. $(x_1,y_1)$ and $(x_3,y_2)$ are two of the hypothetical inliers, while $(x_1,y_4)$ and $(x_3,y_1)$ are two of the outliers.
%    \item If $(x, y)$ is a hypothetical inlier, we collect all other pairs from $\mathcal{D}$ that agree with this hypothetical inlier, forming a set $\mathcal{S}$ called \emph{consensus set}. To find the pairs that agree with $(x, y)$, we first find all test cases that $x$ can pass, denoted as $\mathcal{S}_y$. Then, we find all code solutions that can pass exactly the same test cases as $x$, denoted as $\mathcal{S}_x$. Finally, the consensus set is the set of all pairs that consist of a code solution from $\mathcal{S}_x$ and a test case from $\mathcal{S}_y$, i.e., $\mathcal{S}=\{(x, y)|x\in\mathcal{S}_x, y\in\mathcal{S}_y\}$. For example in Figure \ref{fig:agree}, we can get $\mathcal{S}_x=\{x_1,x_2\}, \mathcal{S}_y=\{y_1,y_2,y_3\}$ from the hypothetical inlier $(x_1,y_1)$ (shown in green box), and $\mathcal{S}_x=\{x_3\}, \mathcal{S}_y=\{y_2,y_3,y_4,y_5\}$ from  $(x_3,y_2)$ (shown in purple box).
%    \item We score the consensus set as $f(\mathcal{S}) = |\mathcal{S}_x||\mathcal{S}_y|$, where $|\mathcal{S}_x|$ is the number of code solutions in $\mathcal{S}_x$ and $|\mathcal{S}_y|$ is the number of test cases in $\mathcal{S}_y$. This score equals to the number of pairs in the consensus set. The intuition is that the more pairs that agree with the hypothetical functionality, the more likely this functionality is correct, according to our assumptions. Following the example in Figure \ref{fig:agree}, the consensus set scores are $6$ and $4$ for the hypothetical inliers $(x_1,y_1)$ and $(x_3,y_2)$, respectively.
%\end{itemize}
%}

\begin{itemize}
    \item We randomly select a pair $(x, y)$ from the set of all possible pairs $\mathcal{D}=\{(x, y)|x\in\mathbf{X}, y\in\mathbf{Y}\}$. We then try to execute the code solution $x$ on the test case $y$. If $x$ can pass $y$, then we say that the pair $(x, y)$ is a \emph{hypothetical inlier}, because it hypothetically describes the correct functionality for the programming problem. Otherwise, we say that $(x, y)$ is an \emph{outlier}, because it fails to describe the correct functionality. Figure \ref{fig:agree} shows a simple example of the programming problem ``return the square of a number''. $(x_1,y_1)$ and $(x_3,y_2)$ are two of the hypothetical inliers, while $(x_1,y_4)$ and $(x_3,y_1)$ are two of the outliers.
    \item If $(x, y)$ is a hypothetical inlier, we collect all other pairs from $\mathcal{D}$ that agree with this hypothetical inlier, forming a set $\mathcal{S}$ called \emph{consensus set}. To find the pairs that agree with $(x, y)$, we first find all test cases that $x$ can pass, denoted as $\mathcal{S}_y$. Then, we find all code solutions that can pass exactly the same test cases as $x$, denoted as $\mathcal{S}_x$. Finally, the consensus set is the set of all pairs that consist of a code solution from $\mathcal{S}_x$ and a test case from $\mathcal{S}_y$, i.e., $\mathcal{S}=\{(x, y)|x\in\mathcal{S}_x, y\in\mathcal{S}_y\}$. For example in Figure \ref{fig:agree}, we can get $\mathcal{S}_x=\{x_1,x_2\}, \mathcal{S}_y=\{y_1,y_2,y_3\}$ from the hypothetical inlier $(x_1,y_1)$ (shown in green box), and $\mathcal{S}_x=\{x_3\}, \mathcal{S}_y=\{y_2,y_3,y_4,y_5\}$ from  $(x_3,y_2)$ (shown in purple box).
    \item We score the consensus set as $f(\mathcal{S}) = |\mathcal{S}_x||\mathcal{S}_y|$, where $|\mathcal{S}_x|$ is the number of code solutions in $\mathcal{S}_x$ and $|\mathcal{S}_y|$ is the number of test cases in $\mathcal{S}_y$. This score is equal to the number of pairs in the consensus set. The intuition is that the more pairs that agree with the hypothetical functionality, the more likely this functionality is correct, according to our assumptions. Following the example in Figure \ref{fig:agree}, the consensus set scores are $6$ and $4$ for the hypothetical inliers $(x_1,y_1)$ and $(x_3,y_2)$, respectively.
\end{itemize}

%There are pairs of the code solutions and the test cases, denoted as $(x, y)$. Some of them are correct to the programming problem (called inliers), while others are incorrect (called outliers). Given all the observed pairs, we propose the dual execution agreement to find the most likely solution, which is based on two assumptions: the incorrect pairs will not agree consistently for any single model and there are enough pairs to agree on a good model. These align to the idea of RANSAC, and we can formulate the dual execution agreement as follows:

%(1) A sample $(x, y)$ is randomly selected. If the code solution $x$ can be executed and pass the test case $y$, then $(x, y)$ is a hypothetical inlier; otherwise, it is an outlier.

%(2) If $(x, y)$ is a hypothetical inlier, we use it to obtain the fitting model $M$. The model is for a kind of functionality. 

%(3) Then we find a consensus set $s$, containing all inliers for the model $M$. Firstly, we find all the test cases that $x$ can pass, denoted as $\mathbf{y}'=\{y'_1,y'_2,{\cdots}\}$. Then, we find all the code solutions that exactly can pass the test cases in $\mathbf{y}'$, denoted as $\mathbf{x}'=\{x'_1,x'_2,{\cdots}\}$. Finally, the consensus set $s=\{(x, y)|x\in\mathbf{x}', y\in\mathbf{y}'\}$.

%(4) We score each consensus set as $f(s) = rg$, where $r$ is the code solution number in $s$ and $g$ is the test case number in $s$.

%The above procedure is repeated many times, each time producing a consensus set with its score. 
%Finally, we get the best code solution $\hat{x}$ by selecting any code solution from the highest scoring consensus set. %\footnote{Some consensus sets may be the same, and we take only one of them.}.
%If we want to obtain $k$ code solutions, we can select one code solution from each of the top $k$ highest scoring unique sets. 
%So far, we have formulated our dual execution agreement aligned with RANSAC, which provides theoretical support to our approach. In fact, the formulation can be simplified to a more intuitive one, as detailed in Appendix \ref{appendix_method}.

%\textcolor{red}{
%We repeat the above procedure for a fixed number of times, each time producing a consensus set with its score. 
%Finally, we get the best code solution $\hat{x}$ by selecting any code solution from the consensus set with the highest score. %\footnote{Some consensus sets may be the same, and we take only one of them.}.
%If we want to obtain $k$ code solutions, we can select one code solution from each of the $k$ consensus sets with the highest scores. 
%So far, we have formulated our dual execution agreement aligned with RANSAC, which provides theoretical support to our approach. In fact, the formulation can be simplified to a more intuitive one, as detailed in Appendix \ref{appendix_method}.}

We repeat the above procedure for a fixed number of times, each time producing a consensus set with its score. 
Finally, we get the best code solution $\hat{x}$ by selecting any code solution from the consensus set with the highest score. %\footnote{Some consensus sets may be the same, and we take only one of them.}.
If we want to obtain $k$ code solutions, we can select the top $k$ consensus sets with the highest scores, and one code solution is picked up from each of the $k$ consensus sets. 
%So far, we have formulated our dual execution agreement aligned with RANSAC, which provides theoretical support to our approach. In fact, the formulation can be simplified to a more intuitive one, as detailed in Appendix \ref{appendix_method}.

%Although we have formulated our dual execution agreement aligned with RANSAC to provide theoretical support, we can also implement it in a simpler way while still following the same intuition. 
%In practice, we can simplify the implementation of the above algorithm by replacing the repeated sampling with enumerating all pairs in $D$, while it still follows the same statistical intuition.
%Specifically, for each code solution $x\in \mathbf{x}$, we run it with all the test cases in $\mathbf{y}$ and record which test cases it can pass. If two code solutions can pass the same set of test cases, then they have the same functionality and we group them together. By doing this, we group all code solutions in $\mathbf{x}$ based on their functionality, denoted as $\mathbf{x}=\{\mathcal{S}_x^1,\mathcal{S}_x^2,{\cdots},\mathcal{S}_x^K\}$, where $K$ is the number of code solution groups. Each group $\mathcal{S}_x$ is associated with a set of test cases that it can pass, denoted by $\mathcal{S}_y$. Then, in total, we obtain $K$ consensus sets, one of which can be denoted as $\mathcal{S}=\{(x, y)|x\in\mathcal{S}_x, y\in\mathcal{S}_y\}$. As before, each consensus set can be scored by $f(\mathcal{S}) = |\mathcal{S}_x||\mathcal{S}_y|$. 
%This implementation differs from the above one by directly finding all consensus sets without iterative sampling. Since the number of code solutions is not extremely huge (at most $1,000$ in our experiments), it is feasible to find all consensus sets, which is the best alternative way to implement the above iterative approach.

%\textcolor{red}{
%To implement the algorithm more efficiently (e.g., reducing the calling times to the large language model $\mathcal{M}$), we use a simplified method that still captures the same  idea. Instead of sampling pairs from $\mathcal{M}$, we examine all possible pairs in $D$. For each code solution $x\in \mathbf{x}$, we run it with every test case in $\mathbf{y}$ and keep track of which test cases it passes. We group together code solutions that pass the same test cases, because they have the same functionality. This way, we divide all code solutions in $\mathbf{x}$ into groups based on their functionality, which we write as $\mathbf{x}=\{\mathcal{S}_x^1,\mathcal{S}_x^2,{\cdots},\mathcal{S}_x^K\}$, where $K$ is the number of groups of code solutions. Each group $\mathcal{S}_x$ has a set of test cases that it passes, which we write as $\mathcal{S}_y$. Then, we get $K$ consensus sets, each of which has the form $\mathcal{S}=\{(x, y)|x\in\mathcal{S}_x, y\in\mathcal{S}_y\}$. We can score each consensus set by $f(\mathcal{S}) = |\mathcal{S}_x||\mathcal{S}_y|$, as before. This method is different from the previous one because it finds all consensus sets right away, without sampling pairs repeatedly. Since the number of code solutions is not very large (at most $1,000$ in our experiments), it is possible to find all consensus sets, which is the best way to implement the previous sampling method.}

In practice, when the number of code solutions in $\mathbf{D}$ is not large, we can simplify the above method by examining all possible pairs in $\mathcal{D}$, instead of sampling pairs from $\mathcal{D}$. Specially, for each code solution $x\in \mathbf{X}$, we run it with every test case in $\mathbf{Y}$ and keep track of which test cases it passes. We group together code solutions that pass the same test cases, because they have the same functionality. This way, we divide all code solutions in $\mathbf{X}$ into groups based on their functionality, which we write as $\mathbf{X}=\{\mathcal{S}_x^1,\mathcal{S}_x^2,{\cdots},\mathcal{S}_x^K\}$, where $K$ is the number of code solution groups. Each group $\mathcal{S}_x$ has a set of test cases that it passes, which we write as $\mathcal{S}_y$. Then, we get $K$ consensus sets, each of which has the form $\mathcal{S}=\{(x, y)|x\in\mathcal{S}_x, y\in\mathcal{S}_y\}$. We can score each consensus set by $f(\mathcal{S}) = |\mathcal{S}_x||\mathcal{S}_y|$, as before. 
This naive version captures the same underline intuition, but it finds all consensus sets right away, without sampling pairs repeatedly.

%\subsection{A Simplified Implementation of Dual Execution Agreement}
%\label{appendix_method}
%We have formulated our dual execution agreement aligned with RANSAC in the above section, which provides theoretical support to our approach. In fact, the formulation can be simplified to a more intuitive one. 
%As mentioned in Section \ref{sec:agree}, in addition to the formulation in line with the RANSAC algorithm, our dual execution agreement can be formulated in a simpler way to answer the question: given the code solutions $\mathbf{x}=\{x_1,x_2,{\cdots},x_N\}$ and the test cases $\mathbf{y}=\{y_1,y_2,{\cdots},y_M\}$ for a certain programming problem, how do we select the solution $\hat{x}$ that is most likely correct? 
%Specially, for each code solution $x\in \mathbf{x}$, we execute it with all the test cases in $\mathbf{y}$. If two code solutions can pass a same set of test cases, 
%then they are sibling solutions with the same functionality; thus, we can put them into the same cluster. In this way, all code solutions in $\mathbf{x}$ can be divided into several clusters, denoted as $\mathbf{x}=\{\mathbf{x}_1,\mathbf{x}_2,{\cdots},\mathbf{x}_K\}$. Let $W=\{w_{ij}\}$ be an $K\times M$ matrix to represent the execution results, where $K$ is the number of code solution clusters and $M$ is the number of test cases. If code solutions in cluster $\mathbf{x}_i$ can pass the test case $y_j$, then $w_{ij}=1$; otherwise, $w_{ij}=0$. 
%The basic idea here is that a good code solution should be agreed upon by both the test cases and the other solutions: (1) The more test cases it can pass, the better the solution is. (2) A larger number of sibling solutions can directly contribute to the correctness of the solution. 
%To keep the notation simple, we also use $\mathbf{x}_i$ and $y_j$ to denote their scores.
%Then, we define the score of each cluster $\mathbf{x}_i$ to be:
%\begin{equation}\label{eq:agree}
%f(\mathbf{x}_i) = N_i^{\frac{1}{2}} \sum_{j=1}^M w_{ij} \cdot g_0(y_j),
%f(\mathbf{x}_i) = r_i \sum_{j=1}^M w_{ij}  g_0(y_j),
%f(\mathbf{x}_i) = |\mathbf{x}_i| \sum_{j=1}^M w_{ij},
%\end{equation}
%where $g_0(y_j)=\frac{1}{M}$ denotes the initial normalized score of test case $y_j$ and $r_i$ 
%where $|\mathbf{x}_i|$ is the code solution number in cluster $\mathbf{x}_i$. This is in line with the idea of Section \ref{sec:agree} that a good code solution can pass the most test cases and agree with the most sibling solutions. 
%$r_i$ is the square root of the code solution number in the cluster $\mathbf{x}_i$. We use the square root to reduce the impact caused by code solutions due to the intuition that the number of code solutions is less important than the number of test cases. For example, there may be one code solution that can pass five test cases, whereas another five code solutions may pass only one test case. We intuitively consider that the former may be more likely correct. 
%Finally, we get the best code solution $\hat{x}$ by selecting any code solution from the highest scoring cluster. %In addition, if we want to obtain $k$ code solutions, we can select one code solution from each of the top $k$ highest scoring clusters.

%\textcolor{red}{
%Although We have formulated our dual execution agreement aligned with RANSAC in the above section to provide theoretical support, we can also implement our dual execution agreement in a simpler way while still following the same intuition. Specifically, for each code solution $x\in \mathbf{x}$, we run it with all the test cases in $\mathbf{y}$ and record which test cases it can pass. If two code solutions can pass the same set of test cases, then they have the same functionality and we group them together. By doing this, we cluster all code solutions in $\mathbf{x}$ based on their functionality, denoted as $\mathbf{x}=\{\mathbf{x}_1,\mathbf{x}_2,{\cdots},\mathbf{x}_K\}$. We use a matrix $W=\{w_{ij}\}$ of size $K\times M$ to store the execution results, where $K$ is the number of code solution clusters and $M$ is the number of test cases. The entry $w_{ij}$ is $1$ if the code solutions in cluster $\mathbf{x}_i$ can pass the test case $y_j$, and $0$ otherwise. 
%Then, we score each cluster $\mathbf{x}_i$ by multiplying the number of code solutions in the cluster, $|\mathbf{x}_i|$, with the number of test cases that the cluster can pass, $\sum_{j=1}^M w_{ij}$. 
%\begin{equation}\label{eq:agree}
%f(\mathbf{x}_i) = |\mathbf{x}_i| \sum_{j=1}^M w_{ij},
%\end{equation}
%This score reflects how well the cluster describes the correct functionality for the programming problem, in line with the idea of Section \ref{sec:agree} that a good code solution can pass the most test cases and agree with the most sibling solutions. Finally, we get the best code solution $\hat{x}$ by choosing any code solution from the cluster with the highest score. If we want to obtain $k$ code solutions, we can choose one code solution from each of the $k$ clusters with the highest scores.
%}

\iffalse
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\textwidth]{fig/agreement-v2.pdf}
    \caption{A simple example of the programming problem ``return the square of a number''. The gray line between a code solution $x$ and a test case $y$ indicates that $x$ can pass $y$, i.e., $(x,y)$ is a hypothetical inlier. The green or purple box indicates a consensus set.}
    \label{fig:agree}
\end{figure}
\fi

%\bei{This basic idea is difficult to maintain, and this may also affect the expression of the main idea in abs and intro:}
%The basic idea of the dual execution agreement is that a good code solution should be agreed upon by both the test cases and the other solutions: (1) The more test cases it can pass, the better the solution is. (2) A larger number of sibling solutions can directly contribute to the correctness of the solution. 





\iffalse
So far, we have introduced the formulation of the dual execution agreement aligned with RANSAC, which provides theoretical support to our approach. In fact, our method can also be formulated in a simpler and more intuitive way. 
All code solutions in $\mathbf{x}$ can be divided into several clusters, denoted as $\mathbf{x}=\{\mathbf{x}_1,\mathbf{x}_2,{\cdots},\mathbf{x}_N\}$. Code solutions in a same cluster are sibling solutions with the same functionality (they can pass a same set of test cases).
Let $w_{ij}$ represent the execution result. If code solutions in cluster $\mathbf{x}_i$ can pass the test case $y_j$, then $w_{ij}=1$; otherwise, $w_{ij}=0$. 
A good code solution should be agreed upon by both the test cases and the other solutions: (1) The more test cases it can pass, the better the solution is. (2) A larger number of sibling solutions can directly contribute to the correctness of the solution. 
%To keep the notation simple, we also use $\mathbf{x}_i$ and $y_j$ to denote their scores.
Hence, we define the score of each cluster $\mathbf{x}_i$ to be:
\begin{equation}\label{eq:agree}
%f(\mathbf{x}_i) = N_i^{\frac{1}{2}} \sum_{j=1}^M w_{ij} \cdot g_0(y_j),
%f(\mathbf{x}_i) = r_i \sum_{j=1}^M w_{ij}  g_0(y_j),
f(\mathbf{x}_i) = |\mathbf{x}_i| \sum_{j=1}^M w_{ij},
\end{equation}
%where $g_0(y_j)=\frac{1}{M}$ denotes the initial normalized score of test case $y_j$ and $r_i$ 
where $|\mathbf{x}_i|$ is the code solution number in cluster $\mathbf{x}_i$. Finally, we get the best code solution $\hat{x}$ by selecting any code solution from the highest scoring cluster. In addition, if we want to obtain $k$ code solutions, we can select one code solution from each of the top $k$ highest scoring clusters.
\fi

\begin{figure}[t]
\begin{minipage}[b]{0.49\linewidth}
\centering
\includegraphics[width=\textwidth]{agreement-v3.pdf}
\caption{A simple example of the programming problem ``return the square of a number''. The gray line between $x$ and $y$ indicates that $x$ can pass $y$, i.e., $(x,y)$ is a hypothetical inlier. The green or purple box indicates a consensus set.}
\label{fig:agree}
\end{minipage}
\hspace{0.1cm}
\begin{minipage}[b]{0.49\linewidth}
\centering
\captionsetup{type=table}
\centering
    \scalebox{0.75}{
        \begin{tabular}{llccc}
        \toprule
        \multicolumn{2}{c}{\textbf{Benchmark}} & \textbf{Problems} & \textbf{GT Tests} & $n$ \\
        \midrule
        \multicolumn{2}{c}{HumanEval} & $164$ & $7.77$ & $100$ \\
        \cmidrule(lr){1-5}
        \multicolumn{2}{c}{MBPP} & $427$ &$3.1$ & $100$\\
        \cmidrule(lr){1-5}
        %\multicolumn{1}{c}{APPS} & $5,000$ &$20.99$ & $50$\\
        \multirow{3}{*}{APPS} & \textsc{Introductory} & $1,000$ & \multirow{3}{*}{$20.99$} & \multirow{3}{*}{$50$}\\
         & \textsc{Interview} & $3,000$ & &\\
         & \textsc{Competition} & $1,000$ & &\\
         \cmidrule(lr){1-5}
        \multicolumn{2}{c}{CodeContests} & $165$ &$203.7$ & $1,000$\\
        \bottomrule
        \end{tabular}
    }
\caption{Statistics of benchmarks: the total number of problems in the benchmark (\emph{Problems}), the average number of ground-truth test cases per problem (\emph{GT Tests}), and the number of sampling code solutions for each problem ($n$).}
\label{tab:benchamrk}
\end{minipage}
\end{figure}


==> CodeT_ Code Generation with Generated Tests (arXiv V2 20221123)/3_experimental_setup.tex <==
\section{Experimental Setup}\label{sec:exp-setup}
%In this section, we introduce the experimental setup, including the pre-trained language models, the benchmarks for code generation, the evaluation metrics, and the implementation details.

\paragraph{Models}
Our experiments are based on Codex \citep{chen2021evaluating}, \incoder \citep{dfried2022incoder} and \codegen \citep{Nijkamp2022ACP}. Codex is a descendant of GPT-3 \citep{brown2020language} and proficient in understanding the provided context and generating functional programs. We use three Codex models with different capabilities provided by OpenAI: {\cushman}, {\davincione}, and {\davincitwo}. 
%\incoder and \codegen are two publicly available pre-trained models. 
\incoder is a unified generative model that can perform left-to-right code generation and code infilling, while \codegen is a family of large-scale language models to perform conversational program synthesis. We take use of the \incoder 6.7B version (\incoderb) and the \codegen 16B Python mono-lingual version (\codegenb).

%Our main experiments are based on Codex \citep{chen2021evaluating}, which is a descendant of GPT-3 \citep{brown2020language}. 
%containing both natural language corpus and publicly available source code in its training data. 
%Codex is proficient in understanding the provided context and generating functional programs, and it has been successfully applied to many programming tasks \citep{drori2021neural, pearce2021can, sarsa2022automatic}.
%We use three Codex models with different capabilities provided by OpenAI: {\cushman}, {\davincione}, and {\davincitwo}.


%Furthermore, we include two publicly available pre-trained models: \incoder \citep{dfried2022incoder} and \codegen \citep{Nijkamp2022ACP}. \incoder is a unified generative model that can perform left-to-right code generation and code infilling (editing) via the causal mask language modelling training objective \citep{armen2022cm3}. 
%The causal mask language modelling objective combines bidirectional context with left-to-right autoregressive language modelling, allowing \incoder to improve performance on both left-to-right code generation and code editing tasks. 
%We use the largest publicly available model with 6 billion parameters.
%\codegen is a family of large-scale language models  trained on natural language and programming data to perform conversational program synthesis. 
%We use its largest publicly available version containing 16 billion parameters.  
%With the scaling up of both pretraining data size and model size,
%conversational programming capacity naturally emerges from the task of autoregressive language modelling.
%We take use of the \incoder 6.7B version (\incoderb) and the \codegen 16B Python mono-lingual version (\codegenb).

\iffalse
\begin{table}[!htbp]
    \centering
    \scalebox{0.9}{
        \begin{tabular}{lccc}
        \toprule
        \multicolumn{1}{c}{\textbf{Benchmark}} & \textbf{Problems} & \textbf{GT Tests} & $n$ \\
        \midrule
        \multicolumn{1}{c}{HumanEval} & $164$ & $7.77$ & $100$ \\
        %\cmidrule(lr){1-5}
        \multicolumn{1}{c}{MBPP} & $427$ &$3.1$ & $100$\\
        \multicolumn{1}{c}{APPS} & $5,000$ &$20.99$ & $50$\\
        %\cmidrule(lr){1-5}
        %\multirow{3}{*}{APPS} & \textsc{Introductory} & $1000$ & \multirow{3}{*}{$20.99$} & \multirow{3}{*}{$50$}\\
       %  & \textsc{Interview} & $3000$ & &\\
       %  & \textsc{Competition} & $1000$ & &\\
       % \cmidrule(lr){1-5}
        \multicolumn{1}{c}{CodeContests} & $165$ &$203.7$ & $1,000$\\
        \bottomrule
        \end{tabular}
    }
    \caption{Statistic numbers of different benchmarks: the total number of problems in the benchmark (\emph{Problems}), the average number of ground-truth test cases per problem (\emph{GT Tests}) and the number of sampling code solutions for each problem ($n$). Specially, APPS includes $1,000$ introductory, $3,000$ interview, and $1,000$ competition level coding problems.  } 
    %\fj{``Problems" denotes the total number of problems in the benchmark. ``GT Tests" denotes the average number of ground-truth test cases per problem, and ``Solutions" denotes the number of sampling code solutions for each problem}.}
    \label{tab:benchamrk}
\end{table}
\fi

\iffalse
\begin{table}[!htbp]
    \centering
    \scalebox{0.9}{
        \begin{tabular}{lcccccc}
        \toprule
        \textbf{Benchmark} & HumanEval & MBPP & APPS \textsc{Introductory} & APPS  \textsc{Interview} & APPS \textsc{Competition} & CodeContests \\
        \midrule
        \textbf{Problems} &  $164$ & $427$ & $1000$ & $3000$ & $1000$ & $165$\\
        \textbf{GT Tests} &  $7.77$ & $3.1$ & \multicolumn{3}{c}{$20.99$} & $203.7$\\
        \textbf{Solutions} & $100$ & $100$ & \multicolumn{3}{c}{$50$} & $1000$\\
        \bottomrule
        \end{tabular}
    }
    \caption{Statistic numbers of different benchmarks. \fj{``Problems" denotes the total number of problems in the benchmark. ``GT Tests" denotes the average number of ground-truth test cases per problem, and ``Solutions" denotes the number of sampling code solutions for each problem}.}
    \label{tab:benchamrk}
\end{table}
\fi

\paragraph{Metrics and Baseline}
We use the metric pass@$k$ (with $n$ samples) for performance evaluation and take advantage of ground truth test cases to determine the functional correctness of code solutions. 
For each problem, we sample $n$ code solutions and then select $k$ of them for evaluation. If any of the $k$ code solutions passes all ground truth test cases, the problem is considered solved. Then pass@$k$ is the percentage of solved problems. 
We use the unbiased definition of pass$@k$ as our baseline \citep{chen2021evaluating}, where $k$ solutions are randomly picked from $n$ samples. Our CodeT uses a dual execution agreement mechanism to select $k$ solutions from $n$ samples, as mentioned in \ref{sec:agree}. 
In addition, we include a clustering method from \cite{li2022competition} for comparison, denoted as AlphaCode-C. Our replication is to use the test inputs generated by \ours, run the solutions on the test inputs, group the solutions by test outputs, and rank the clusters by size (details in Appendix \ref{appendix_simplecount}). %We also introduce a post-processing method to further improve its performance (details in Appendix \ref{appendix_simplecount}).

%For each problem, $k$ code solutions are produced as the final result. If any of the $k$ code solutions passes all ground truth test cases, the problem is considered solved. Then pass@$k$ is the percentage of solved problems. Following \cite{chen2021evaluating}, pass@$k$ can be formulated as:
%\begin{equation}
	%{\rm{pass@}}k:=\expectation_{\rm{Problems}}\left[1-h(k)\right],
	%{\rm{pass@}}k:=\expectation_{\rm{Problems}}\left[1-\frac{\tbinom{n-c}{k}}{\tbinom{n}{k}}\right],
%	{\rm{pass@}}k:=\expectation_{\rm{Problems}}\left[1-{\tbinom{n-c}{k}}/{\tbinom{n}{k}}\right],
%\end{equation}
%where $n\geq k$ is the sampling number and $c\leq n$ is the number of correct code solutions. 
%where $h(k)$ is the probability that none of the $k$ code solutions can pass all ground-truth test cases. 
%For the baseline method, $n$ code solutions are sampled. For \ours, we selected the top $k$ code solutions as mentioned in Section \ref{sec:agree}.

%so $h(k)$ is calculated by $h(k)=\tbinom{n-c}{k}/\tbinom{n}{k}$ following \cite{chen2021evaluating}, where $n\geq k$ is the sampling number ($n=100$ in our implementation) and $c\leq n$ is the number of correct code solutions. 
%By \ours, we get $k$ code solution clusters with top scores for each problem, denoted as $(\mathbf{x}_1,\mathbf{x}_2,{\cdots},\mathbf{x}_k)$.
%Then $h(k)$ can be calculated as $h(k)=\prod_{i=1}^{k} (n_i-c_i)/n_i$, where $n_i$ is the number of total code solutions in cluster $\mathbf{x}_i$ and $c_i$ is the number of correct code solutions in cluster $\mathbf{x}_i$. 

%Note that $i-1=(j-1) \bmod N$, which is designed for the cases that the cluster number $N<k$. In addition, we merge the clusters with the same score at first.

%\fj{The baseline method we use for comparison is to randomly pick $k$ code solutions from $n$ samples per problem. In addition, we also include a clustering method used in AlphaCode\citep{li2022competition} for comparison, denoted as AlphaCode-C. It first groups together the semantically equivalent code solutions and then picks the solutions in order of cluster size. However, this method relies on an additional test input generation model, which is hard and expensive to replicate. Finally, we implemented AlphaCode-C using the test cases generated by \ours and introduced a post-processing method to further improve its performance. A detailed introduction of AlphaCode-C can be found in Appendix. XX.}


%Following previous studies \citep{hendrycks2021measuring, chen2021evaluating, austin2021program}, we take advantage of ground truth test cases to determine the functional correctness of code solutions. % and employ ``strict accuracy'' as the evaluation metric, which is the percentage of problems solved by the generated solutions.
%For baseline methods, we use the metric pass@$k$ to evaluate the performance. $k$ code solutions are generated per problem, and a problem is considered solved if any of the generated code solutions passes all ground truth test cases. Then pass@$k$ is the percentage of solved problems. In our implementation, we calculate pass@$k$ using the method introduced by \cite{chen2021evaluating}:
%\begin{equation}
%	{\rm{pass@}}k:=\expectation_{\rm{problems}}\left[1-\frac{\tbinom{n-c}{k}}{\tbinom{n}{k}}\right],
%\end{equation}
%where $n\geq k$ is the sampling number and $c\leq n$ is the number of correct code solutions. In the experiments, we use $n=100$.


%When sampling $n$ code solutions for each problem, pass@$k$ calculates the unbiased estimate of the solved problem percentage by randomly picking $k$ ($k\leq n$) from $n$ samples per task.

%In this paper, we introduce the metric \passattopk to handle the situation where the generated code solutions are ranked. By \ours, we get the code solution clusters with descending scores for each problem, denoted as $(\mathbf{x}_1,\mathbf{x}_2,{\cdots},\mathbf{x}_N)$, where $\mathbf{x}_i>\mathbf{x}_j$ if $i<j$. The \passattopk is defined as:
%\begin{equation}
%	{\rm{pass@top}}\text -k:=\expectation_{\mathrm{problems}}\left[1-\prod_{j=1}^{k} \frac{n_i-c_i}{n_i}\right],
%\end{equation}
%where $n_i$ is the number of code solutions in cluster $\mathbf{x}_i$ and $c_i$ is the number of correct code solutions in cluster $\mathbf{x}_i$.  Note that $i-1=(j-1) \bmod N$, which is designed for the cases that the cluster number $N<k$. In addition, we merge the clusters with the same score at first.

%Given the generated code solution clusters $\mathbf{x}$, we first merge the clusters with the same ranking and get the ranked clusters $\mathbf{s}=\{\mathbf{s}_1,\mathbf{s}_2,{\cdots},\mathbf{s}_L\}$. If $L<k$, we will do a repeat sampling to fill $\mathbf{s}$ up to $k$ clusters by having $\mathbf{s}_{i}:=\mathbf{s}_{1+(i-1)\bmod L},1\leq i\leq k$. Finally we can get the unbiased estimator
%\begin{equation}
%	\mathrm{pass@}top\text -k:=\expectation_{\mathrm{problems}}\left[1-\prod_{l=1}^{k}P_w(s_i)\right],
%\end{equation}
%where $P_w(s_i)$ is the probability of picking out a wrong solution from cluster $s_i$,
%\begin{equation}
%	P_w(s_i):=\frac{\countif\limits_{x_j\in s_i} (x_{j}\mathrm{\ is\ wrong})}{\#(s_i)}.
%\end{equation}
%To keep the notation simple, we also use pass@$k$ to represent the \passattopk results of our methods. 

\paragraph{Benchmarks}
\label{benckmarks}
We conduct experiments on four public code generation benchmarks in the zero-shot setting. The statistics of benchmarks are shown in Table \ref{tab:benchamrk}. (1) {\bf HumanEval}~\citep{chen2021evaluating} consists of hand-written Python programming problems. %, each with a canonical solution and several ground truth test cases. 
The original contexts include example input-output cases, which are removed in our experiments to avoid exposing real test cases. The experiment in Appendix \ref{sec:appendix_origial_humaneval} shows that this removal operation is reasonable and indispensable. 
(2) {\bf MBPP}~\citep{austin2021program} (sanitized version) contains crowd-sourced Python programming problems, and we follow HumanEval to construct the context for it. %, which contains a well-formed function header and its natural language description in the form of a multi-line comment.
(3) {\bf APPS}~\citep{hendrycks2021measuring} consists of coding problems collected from open-access coding websites, which have different difficulty levels.
(4) {\bf CodeContests}~\citep{li2022competition} includes competitive programming problems scraped from the Codeforces platform. %The construction of the context is the same as for APPS.
To enable zero-shot inference, we construct the context for APPS and CodeContests as follows: the original problem description is treated as a comment where input-output examples are removed, and a simple function header ``{${\rm def}$ $\rm{ solution(stdin: str) \rightarrow str:}$}'' is placed after the comment to accommodate the input/output data format. More implementation details can be found in Appendix \ref{sec:appendix_detail}.

%We conduct experiments on two public code generation benchmarks using zero-shot settings. 
%Code generation is based on the context to generate code solutions, and test case generation is based on the context and the instruction (as mentioned in Section \ref{sec:testcase}) to generate test cases.

%{\bf{HumanEval}} is a code generation benchmark consisting of $164$ hand-written Python programming problems, covering subjects of language comprehension, reasoning, algorithms, and simple mathematics~\citep{chen2021evaluating}. As shown in Figure \ref{fig:prelimilary}, the context of each problem may include the natural language description in the form of a comment, a function header, and statements like imports. Each problem includes a canonical solution and several ground truth test cases. To be clear, the original context of each problem may include example input-output cases, which are removed in our experiments to avoid exposing real test cases.% during test case generation. 

%{\bf{MBPP}} (sanitized version) contains $427$ crowd-sourced Python programming problems, ranging from the basic usage of standard library functions to problems that require nontrivial external knowledge~\citep{austin2021program}. 
%Originally, each problem includes the natural language problem description, a function header, a canonical solution, and several ground truth test cases. We follow HumanEval to construct the context for MBPP, which contains a well-formed function header and its natural language description in the form of a multi-line comment.

%MBPP\footnote{There are two versions of the MBPP benchmark, a larger dataset having 974 problems and a smaller dataset having 427 sanitized problems. In this study, we use the sanitized version since the authors\citep{austin2021program} claim that it is of higher quality.}
%\bigbenchppc\footnote{\bigbenchppc denotes the \href{https://github.com/google/BIG-bench/blob/main/bigbench/benchmark_tasks/python_programming_challenge/README.md}{python programming challenge} task introduced in BIG-bench\citep{srivastava2022beyond}.}\citep{srivastava2022beyond}. 
%All the three benchmarks are proposed to evaluate the function-level code generation ability of models with the given context. 
%(3) The \bigbenchppc dataset is rather small, containing 32 Python problems that vary in difficulty. Each of them includes a function signature, a two-line comment that describes the problem and the types of arguments, and a number of ground truth test cases.

% For MBPP, we build two variants of prompt formats, namely MBPP-NL and MBPP-HM. In terms of MBPP-NL, we concatenate the problem description and the name of entry point function as the input prompt\footnote{For example, the problem description is ``Write a python function to sort the given array by using merge sort''. We will append the description with a short hint ``The function name is merge\_sort'' to facilitate extracting entry point functions from generated code samples.}. While MBPP-HM follows the prompt format of HumanEval, having a well-formed function signature and the natural language description in multi-line comment.
%(3) For \bigbenchppc, we keep the input prompt format unchanged, which contains a two-line comment and a function signature.

%To perform zero-shot test case generation, we simply append an instruction (introduced in Section \ref{preliminary}) to the code generation prompt. Specially, we remove the example input-output cases in the docstring bodies of HumanEval when generating test cases to prevent ground truth leakage.
% Moreover, there is no need for the ``${\rm{pass}}$'' placeholder when adapting MBPP-NL to test case generation since no function headers are provided.



%\paragraph{Implementation Details}
%\label{sec:implementation_details}

%For experiments with Codex models, we set the top $p$ to $0.95$ and the max generation length to $300$. To get the results of baseline pass@$1$, the temperature is set to $0$ and the sampling number $n$ is set to $1$. For other results, the temperature is set to $0.8$ and the sampling number $n$ is set to $100$ for HumanEval/MBPP, $50$ for APPS and $1000$ for CodeContests. That is, for baseline pass@$k$ ($k>1$), we use sampling number $n$; for \ours, we select the top $k$ code solutions as mentioned in Section \ref{sec:agree} and use $n=k$. The timeout of executing a test case is set to $0.1$ seconds. For code solution post-processing, we follow \cite{chen2021evaluating} to truncate the generated content by five stop sequences: ``\textbackslash${\rm nclass}$", ``\textbackslash${\rm ndef}$", ``\textbackslash ${\rm n}$\#", ``\textbackslash${\rm nif}$", and ``\textbackslash${\rm nprint}$". For test case post-processing, we extract the first five assertions that conform to the Python syntax for each generated sample. A valid assertion should start with ``${\rm assert}$" and contain the name of the corresponding entry point function. For experiments with \incoder and \codegen, we use the HuggingFace transformers library \citep{Wolf2019HuggingFacesTS}. The setup and post-processing procedure are the same as in the Codex experiments, except that the baseline pass@$1$ results are obtained by picking the sample with the highest mean log-probability from $n=100$ samples with a small temperature close to $0$. To speed up our experiments, we run both models with half precision. In the implementation, when scoring consensus sets in \ours, we use the square root of $|\mathcal{S}_x|$ to reduce the impact caused by code solutions. A supporting experiment can be found in Appendix \ref{appendix_sqrt}. 

% the short version
%To get the results of baseline pass@$1$, the temperature is set to $0$ and the sampling number $n$ is set to $1$. For other results, the temperature is set to $0.8$ and the sampling number $n$ is set to $100$ for HumanEval/MBPP, $50$ for APPS, and $1,000$ for CodeContests. That is, for baseline pass@$k$, we use sampling number $n$; for \ours, we select the top $k$ code solutions as mentioned in Section \ref{sec:agree} and use $n=k$. We set the top $p$ to $0.95$, the max generation length to $300$, and the timeout of executing a test case to $0.1$ seconds. For each test case sample, we extract the first five valid assertions. When scoring consensus sets in \ours, we use the square root of $|\mathcal{S}_x|$ to reduce the impact caused by code solutions. A supporting experiment can be found in Appendix \ref{appendix_sqrt}. More implementation and post-processing details can be found in Appendix \ref{sec:appendix_details}.

%To get the results of baseline pass@$1$, we use the greedy search setting where the temperature is set to $0$, and the sampling number $n$ is set to $1$. For other results, the temperature is set to $0.8$, and the sampling number $n$ is set to $100$ for HumanEval/MBPP, $50$ for APPS, and $1,000$ for CodeContests. That is, to calculate the baseline pass@$k$, we use the sampling number $n$; for \ours, we select the top $k$ code solutions as mentioned in Section \ref{sec:agree} and use $n=k$. 




%\fj{We also notice that duplications exist in the generated code solutions and test cases. We perform an ablation study in Appendix \ref{appendix_dedup} to show that de-duplication has little influence on the results of \ours. Moreover, we discuss the sensitivity of \ours to the temperature in Appendix \ref{appendix_temperature}, showing the rationality of choosing a rather high temperature of $0.8$.})



%For experiments with \incoder and \codegen models, we use the same setup and post-processing procedure as the Codex experiments except following details. First, we select \incoder 6.7B version (\incoderb) and \codegen 16B Python mono-lingual version (\codegenb) to perform code and test case generation using HuggingFace transformers library \citep{Wolf2019HuggingFacesTS}. Second, to speed up our experiments, we run both models in half precision. We also follow \cite{chen2021evaluating} to pick the sample with highest mean log-probability from $n=100$ samples to get the results of pass@1 baseline. 
%while no details have yet been made public on how OpenAI API implements single sample selection from Codex models.


%\textbf{post-processing for code solutions: }Though we provide Codex with function headers when generating code solutions, the model will continue producing additional functions or statements. We follow \citep{chen2021evaluating} to truncate the generated content by five stop sequences: `\textbackslash nclass', `\textbackslash ndef', `\textbackslash n\#', `\textbackslash nif', or ‘\textbackslash nprint’. 
% For the MBPP-NL dataset that provides no function headers, we will simply extract the entry point function body between the function signature and the stop token `\textbackslash n\textbackslash n' from the generated content.

%\textbf{post-processing for test cases: }Our special designed instruction for test case generation ends with the `assert' keyword, which helps alleviate the effort of post-processing. Specifically, we extract the one-line/multi-line assertions\footnote{A valid assertion should start with `assert' and contain the name of entry point function. For example, ``assert merge\_sort([2,3,1]) == [1,2,3]''.} that conform to the Python syntax from generated content. 


==> CodeT_ Code Generation with Generated Tests (arXiv V2 20221123)/4_experimental_results.tex <==
\section{Experimental Results}\label{sec:exp_res}

In this section, we evaluate \ours on five different pre-trained models and four benchmarks to verify its effectiveness, followed by test case analysis and case studies to provide more insights.
%a deep analysis on test cases and case studies%and different design choices in \ours. We also show some case studies to provide more insights. We also show some case studies to provide more insights.

\begin{table}[t]
    \centering
    \scalebox{0.85}{
        \begin{tabular}{llllllllll}
        \toprule
        \multicolumn{1}{c}{{\textbf{Methods}}} & \multicolumn{3}{c}{{\textbf{Baseline}}} & \multicolumn{3}{c}{{\textbf{AlphaCode-C}}} & \multicolumn{3}{c}{{\textbf{\ours}}} \\
        \cmidrule(lr){1-1}
        \cmidrule(lr){2-4}
        \cmidrule(lr){5-7}
        \cmidrule(lr){8-10}
        \multicolumn{1}{c}{$k$}&\multicolumn{1}{c}{$1$} & \multicolumn{1}{c}{$10$} & \multicolumn{1}{c}{$100$} & \multicolumn{1}{c}{$1$} &\multicolumn{1}{c}{$2$} & \multicolumn{1}{c}{$10$} & \multicolumn{1}{c}{$1$} &\multicolumn{1}{c}{$2$} & \multicolumn{1}{c}{$10$}\\
        \midrule
        \grayline \multicolumn{10}{c}{\textbf{HumanEval}}\\
        \cushman & \colorblue $33.5$ & \coloryellow $54.3$ & $77.4$ & $39.6$ & $46.4$ & $63.8$ & \colorblue$44.5$~\improve{11.0} & $50.1$ & \coloryellow$65.7$~\improve{11.4}\\
        %\midrule
         \davincione & \colorblue$39.0$ & \coloryellow$60.6$ & $84.1$ & $41.6$ & $50.7$ & $75.6$ & \colorblue$50.2$~\improve{11.2} & $58.9$ & \coloryellow$75.8$~\improve{15.2}  \\
        %\midrule
         \davincitwo & \colorblue$47.0$ &\coloryellow $74.9$ & $92.1$ & $55.1$ & $64.1$ & $84.4$ & \colorblue$65.8$~\improve{18.8} & $75.1$ & \coloryellow$86.6$~\improve{11.7}  \\
         %\incoderorig & $15.2$ & $27.8$ & $47.0$ &$-$&$-$&$-$ \\
        %\midrule
         %\codegenorig & $29.3$ & $49.9$ & $75.0$ &$-$&$-$&$-$  \\
         \incoderb & \colorblue $16.4$~\originalres{15.2} & \coloryellow $28.3$~\originalres{27.8} & $47.5$~\originalres{47.0} & $17.7$ & $23.8$ & $34.8$ & \colorblue $20.6$~\improve{4.2} & $27.6$ & \coloryellow $37.1$~\improve{8.8}  \\
         \codegenb & \colorblue $29.7$~\originalres{29.3} & \coloryellow $50.3$~\originalres{49.9} & $73.7$~\originalres{75.0} & $27.3$ & $38.5$ & $64.4$ & \colorblue $36.7$~\improve{7.0} & $44.7$ & \coloryellow $59.3$~\improve{9.0} \\
        \midrule
        \grayline \multicolumn{10}{c}{\textbf{MBPP}}\\
        \cushman & \colorblue$45.9$ & \coloryellow$66.9$ & $79.9$ & $51.5$ & $59.0$ & $73.3$ & \colorblue$55.4$~\improve{9.5} & $61.7$ & \coloryellow$72.7$~\improve{5.8}  \\
         \davincione & \colorblue $51.8$ & \coloryellow$72.8$ & $84.1$ & $56.2$ & $64.7$ & $78.8$ & \colorblue$61.9$~\improve{10.1} & $69.1$ & \coloryellow$79.3$~\improve{6.5}  \\
         \davincitwo & \colorblue$58.1$ &\coloryellow $76.7$ & $84.5$ & $62.0$ & $70.7$ & $79.9$ & \colorblue$67.7$~\improve{9.6} & $74.6$ & \coloryellow$81.5$~\improve{4.8} \\
         %\incoderorig & $19.4$&$-$&$-$&$-$&$-$&$-$ \\
         \incoderb & \colorblue $21.3$~\originalres{19.4} & \coloryellow $46.5$ & $66.2$ & $26.7$ & $35.3$ & $56.2$ & \colorblue $34.4$~\improve{13.1} & $43.9$ & \coloryellow $58.2$~\improve{11.7}   \\
         \codegenb & \colorblue $42.4$ & \coloryellow $65.8$ & $79.1$ & $41.0$ & $55.9$ & $73.6$ & \colorblue $49.5$~\improve{7.1} & $56.6$ & \coloryellow $68.5$~\improve{2.7}   \\
        \bottomrule
        \end{tabular}
    }
    \caption{Pass@$k$ ($\%$) on the HumanEval and MBPP benchmarks. AlphaCode-C is our replication of the clustering method in \cite{li2022competition}. The numbers in {\textcolor{red}{red}} indicate the absolute improvements of \ours over baseline on pass@$1$ and pass@$10$. 
    We also list the baseline results from \cite{dfried2022incoder} and \cite{Nijkamp2022ACP} for reference in {\textcolor{gray}{gray}}, where the settings of context are not exactly the same as ours.
    %For baseline pass@$1$, the temperature is set to $0$ and sampling number is set to $1$; for others, temperature is set to $0.8$ and sampling number is set to $100$. 
    For \ours, temperature is set to $0.8$ and sampling number is set to $100$. 
    We do not show \ours pass@$100$, since it is the same as the baseline pass@$100$.
    }
    \label{tab:main}
\end{table}


\subsection{Results on HumanEval and MBPP}

\label{sec:mainres}
The experimental results of various models on the HumanEval and MBPP benchmarks are summarized in Table \ref{tab:main}. 
%The baseline pass@$1$ results are obtained by setting the Codex temperature to $0$ and sampling only $1$ code solution, since lower temperature results in higher pass@$1$. For baseline pass@$10$ and pass@$100$, we set the temperature to $0.8$ and generate $100$ code solutions. 
%Using HumanEval in the Baseline column as an example, we find our reproduced results of the 12B code-cushman-001 model are slightly better than that of the Codex-12B model reported in the original Codex paper \citep{chen2021evaluating} ($33.5\%$ vs. $28.6\%$ in pass@$1$ and $77.4\%$ vs. $72.3\%$ in pass@$100$). We conjecture that code-cushman-001 is a better 12B pre-trained model than the original Codex-12B model. On the other hand, if we compare the pass@$100$ to pass@$1$, it is clear that the former is significantly better than the latter, indicating the potential to select the best code solution from the $100$ generated samples. 
If we compare the pass@$100$ to pass@$1$ on the Baseline column, it is clear that the former is significantly better than the latter, indicating the potential to select the best code solution from the $100$ generated samples. 
%\ours is performed on the $100$ generated code solutions, so the baseline pass@$100$ is the ceiling of \ours's performance. 

For three Codex models, when we compare the \ours column with the Baseline column, \ours pass@$1$ achieves an absolute improvement of about $10\%$ over the baseline pass@$1$. The improvements are consistently above $10\%$ on HumanEval. Surprisingly, even for the strongest baseline, code-davinci-002, the improvement is $18.8\%$, boosting the pass@$1$ to $65.8\%$, which is a $20$+$\%$ absolute improvement over the best previously reported results~\citep{inala2022fault}. We attribute this larger improvement to the higher quality of test cases generated by code-davinci-002, providing a deeper analysis in Section \ref{sec:exp_test}. 
\ours also achieves exceptional performance on the MBPP benchmark, although the magnitude of the improvements is slightly less than that of HumanEval. Using the code-davinci-002 as an example, the pass@$1$ improves by $9.6\%$.  
%It can be observed that most pass@$1$ results have an absolute improvement of about $10\%$ over the baseline, demonstrating the effectiveness of \ours on selecting the best code solution. For \davincitwo on the HumanEval benchmark, the improvement surprisingly reaches $18.8\%$. 
We also report \passattop{2} and \passattop{10} of \ours to further show its superiority. The \passattop{2} results of \ours are close to the baseline pass@$10$ results. Meanwhile, the improvements on pass@$10$ are also consistently over $10\%$ on the HumanEval benchmark. %Since \ours is performed on the $100$ generated code solutions, its pass@$100$ performance is the same as that of the baseline. 
%In addition, we perform an ablation study in Appendix \ref{appendix_simplecount}, where only the number of code solutions or test cases is considered to score a consensus set, demonstrating the plausibility of our dual execution agreement.

The experimental results of \incoderb and \codegenb further verify the effectiveness of \ours.
It is obvious \ours can significantly improve the pass@$1$, with absolute improvements in the range of $4.2\%$ to $13.1\%$. \incoderb achieves the greatest improvement with a gain of $13.1\%$ on the MBPP benchmark. Similar to the experimental results of Codex, the \passattop{2} results are close to the baseline pass@$10$. All the results demonstrate that \ours can boost the performance of various pre-trained language models consistently. 

%\fj{As for AlphaCode-C, it outperforms the Baseline on both benchmarks, demonstrating the effectiveness of clustering code solutions based on their functionality, which conforms to our finding in Appendix \ref{appendix_simplecount}. However, \ours can consistently outperform AlphaCode-C, especially when using more powerful code generation models (i.e., \davincione and \davincitwo), showing the superiority of dual execution agreement.}
As for AlphaCode-C, it is consistently inferior to \ours on both benchmarks using different models, demonstrating the superiority of our dual execution agreement that takes test case information into consideration.
In addition, we notice that duplication exists in the generated code solutions and test cases. We perform an ablation study in Appendix \ref{appendix_dedup} to show that de-duplication has little influence on the results of \ours. Moreover, we discuss the sensitivity of \ours to the temperature in Appendix \ref{appendix_temperature}, showing the rationality of choosing a rather high temperature at $0.8$.

%\fj{More supplementary experiments can be found in Appendix \ref{appendix_simplecount}, where we build another baseline that rank the code solutions by simply count their passed test cases, and we evaluate the performance of \ours on the original HumanEval benchmark. (with the example input-output cases in the problem descriptions untouched) }

%In addition, we compare the performance between \oursiter and \ours. The results show that they are comparable without any significant difference.  We conjecture it might be unnecessary to consider the importance of test cases in this way, or an obviously good test case with a high score can pass many different solutions without introducing differentiation to rank the code solutions. We will leave the further study of a more complicated iterative approach for future work. 
%and these  be  can benefit the scores of many code solutions, but has less impact on the ranking of code solutions.  
\iffalse
\begin{table}[t]
    \centering
    \scalebox{0.9}{
        \begin{tabular}{lllllll}
        \toprule
        \multicolumn{1}{c}{{\textbf{Methods}}} & \multicolumn{3}{c}{{\textbf{Baseline}}} & \multicolumn{3}{c}{{\textbf{\ours}}}\\
        \cmidrule(lr){1-1}
        \cmidrule(lr){2-4}
        \cmidrule(lr){5-7}
        \multicolumn{1}{c}{$k$}&\multicolumn{1}{c}{$1$} & \multicolumn{1}{c}{$10$} & \multicolumn{1}{c}{$100$} & \multicolumn{1}{c}{$1$} &\multicolumn{1}{c}{$2$} & \multicolumn{1}{c}{$10$}\\
        \midrule
        \grayline \multicolumn{7}{c}{\textbf{HumanEval}}\\
        \cushman & \colorblue $33.5$ & \coloryellow $54.3$ & $77.4$ & \colorblue$44.5$~\improve{11.0} & $50.1$ & \coloryellow$65.7$~\improve{11.4} \\
        %\midrule
         \davincione & \colorblue$39.0$ & \coloryellow$60.6$ & $84.1$ & \colorblue$50.2$~\improve{11.2} & $58.9$ & \coloryellow$75.8$~\improve{15.2} \\
        %\midrule
         \davincitwo & \colorblue$47.0$ &\coloryellow $74.9$ & $92.1$ & \colorblue$65.8$~\improve{18.8} & $75.1$ & \coloryellow$86.6$~\improve{11.7} \\
         %\incoderorig & $15.2$ & $27.8$ & $47.0$ &$-$&$-$&$-$ \\
        %\midrule
         %\codegenorig & $29.3$ & $49.9$ & $75.0$ &$-$&$-$&$-$  \\
         \incoderb & \colorblue $16.4$~\originalres{15.2} & \coloryellow $28.3$~\originalres{27.8} & $47.5$~\originalres{47.0} & \colorblue $20.6$~\improve{4.2} & $27.6$ & \coloryellow $37.1$~\improve{8.8} \\
         \codegenb & \colorblue $29.7$~\originalres{29.3} & \coloryellow $50.3$~\originalres{49.9} & $73.7$~\originalres{75.0} & \colorblue $36.7$~\improve{7.0} & $44.7$ & \coloryellow $59.3$~\improve{9.0}\\
        \midrule
        \grayline \multicolumn{7}{c}{\textbf{MBPP}}\\
        \cushman & \colorblue$45.9$ & \coloryellow$66.9$ & $79.9$ & \colorblue$55.4$~\improve{9.5} & $61.7$ & \coloryellow$72.7$~\improve{5.8} \\
         \davincione & \colorblue $51.8$ & \coloryellow$72.8$ & $84.1$ & \colorblue$61.9$~\improve{10.1} & $69.1$ & \coloryellow$79.3$~\improve{6.5} \\
         \davincitwo & \colorblue$58.1$ &\coloryellow $76.7$ & $84.5$ & \colorblue$67.7$~\improve{9.6} & $74.6$ & \coloryellow$81.5$~\improve{4.8}\\
         %\incoderorig & $19.4$&$-$&$-$&$-$&$-$&$-$ \\
         \incoderb & \colorblue $21.3$~\originalres{19.4} & \coloryellow $46.5$ & $66.2$ & \colorblue $34.4$~\improve{13.1} & $43.9$ & \coloryellow $58.2$~\improve{11.7}  \\
         \codegenb & \colorblue $42.4$ & \coloryellow $65.8$ & $79.1$ & \colorblue $49.5$~\improve{7.1} & $56.6$ & \coloryellow $68.5$~\improve{2.7}  \\
        \bottomrule
        \end{tabular}
    }
    \caption{Pass@$k$ ($\%$) on the HumanEval and MBPP benchmarks. The numbers in {\textcolor{red}{red}} indicate the absolute improvements of \ours over baseline on pass@$1$ and pass@$10$. 
    We also list the baseline results from \cite{dfried2022incoder} and \cite{Nijkamp2022ACP} for reference in {\textcolor{gray}{gray}}, where the settings of context are not exactly the same as ours.
    %For baseline pass@$1$, the temperature is set to $0$ and sampling number is set to $1$; for others, temperature is set to $0.8$ and sampling number is set to $100$. 
    \fj{For \ours, temperature is set to $0.8$ and sampling number is set to $100$. }
    We do not show \ours pass@$100$, since it is the same as the baseline pass@$100$.
    }
    \label{tab:main}
\end{table}
\fi


\begin{table}[t]
    \centering
    \scalebox{0.93}{
        \begin{tabular}{lllllllllll}
        \toprule
        \multicolumn{2}{c}{{\textbf{Methods}}} & \multicolumn{5}{c}{{\textbf{Baseline}}} & \multicolumn{4}{c}{{\textbf{\ours}}}\\
        \cmidrule(lr){1-2}
        \cmidrule(lr){3-7}
        \cmidrule(lr){8-11}
        \multicolumn{2}{c}{$k$}&\multicolumn{1}{c}{$1$} & \multicolumn{1}{c}{$10$} &
        \multicolumn{1}{c}{$50$} &\multicolumn{1}{c}{$100$} &
        \multicolumn{1}{c}{$1000$} &\multicolumn{1}{c}{$1$} &\multicolumn{1}{c}{$2$} &
        \multicolumn{1}{c}{$10$} &\multicolumn{1}{c}{$100$}\\
        \midrule
        \multirow{3}{*}{APPS} & \textsc{Introductory} &\colorblue $27.2$&\coloryellow $46.6$&$59.4$&-&-&\colorblue $34.6$~\improve{7.4}& $41.2$&\coloryellow $53.2$~\improve{6.6}&-\\
        & \textsc{Interview} &\colorblue $5.1$&\coloryellow $12.8$&$23.0$&-&-&\colorblue $8.1$~\improve{3.0}&$11.2$&\coloryellow $18.1$~\improve{5.3}&-\\
        & \textsc{Competition}&\colorblue $1.8$&\coloryellow $4.9$&$12.1$&-&-&\colorblue $2.2$~\improve{0.4}&$4.1$&\coloryellow $8.6$~\improve{3.7}&-\\
        % \midrule
        \cmidrule(lr){1-11}
        \multicolumn{2}{c}{CodeContests} &\colorblue $0.7$ & \coloryellow $3.0$ & $5.7$ &\colorgreen $7.5$ & $13.9$ & \colorblue $2.1$~\improve{1.4} & $2.3$ & \coloryellow $5.3$~\improve{2.3} & \colorgreen $9.9$~\improve{2.4} \\
        \bottomrule
        \end{tabular}
    }
    \caption{Pass@$k$ ($\%$) results on the APPS and CodeContests benchmarks using \davincitwo in the zero-shot setting. The numbers in {\textcolor{red}{red}} indicate the absolute improvements of \ours over baseline on pass@$1$, pass@$10$ and pass@$100$. 
    For \ours, temperature is set to $0.8$ and sampling number is set to $50$ for APPS and $1,000$ for CodeContests. 
    }
    \label{tab:apps_code}
\end{table}

\subsection{Results on APPS and CodeContests}
\label{sec:exp_apps_codecontests}

We also conduct experiments on two more challenging benchmarks, APPS and CodeContests. We build the zero-shot versions of APPS and CodeContests to be in line with our setting of HumanEval and MBPP by removing the example input-output cases in the problem descriptions. We employ \davincitwo for code solution and test case generation. The sampling number is set to $50$ for APPS to save computation cost on the $5,000$ testing problems, while for CodeContests, following \cite{li2022competition}, the sampling number is set to $1,000$ to solve especially hard problems. 
From the results summarized in Table \ref{tab:apps_code}, we can clearly observe the consistent performance improvements on both benchmarks using \ours. 
The absolute pass@$1$ improvement is $7.4\%$ for introductory problems in APPS, while the improvements are not significant for competition level problems in APPS and CodeContest, indicating their difficulties.
%We can achieve competitive and even better performance with the zero-shot setting compared to some previously reported results using few-shot prompts and model fine-tuning )~\citep{chen2021evaluating, hendrycks2021measuring, li2022competition}. 
In addition, we notice that \davincitwo may generate many trivial code solutions for the problems in APPS and CodeContests due to the superior difficulty of these two benchmarks. We perform a comprehensive study in Appendix \ref{appendix_remove_trivial} to demonstrate the robustness of \ours to this issue.
Inspired by \cite{chen2021evaluating} and \cite{li2022competition}, we also conduct experiments in the one-shot setting, which is detailed in Appendix \ref{appendix_oneshot}.
%\fj{Specially, we notice that \davincitwo may generate many trivial code solutions for the problems in APPS and CodeContests due to the superior difficulty of the two benchmarks. We perform a comprehensive study in Appendix \ref{appendix_remove_trivial} to demonstrate the robustness of \ours for this issue.
%Inspired by \cite{chen2021evaluating} and \cite{li2022competition}, we also conduct experiments with the one-shot setting, which is detailed in Appendix \ref{appendix_oneshot}.}

\iffalse
\begin{table}[t]
    \centering
    \scalebox{0.98}{
        \begin{tabular}{lccc}
        \toprule
        & \textsc{Introductory} & \textsc{Interview} & \textsc{Competition} \\
        \midrule
        Baseline \passattop{1} & \colorblue $27.2$ & \colorblue $5.1$ & \colorblue $1.8$ \\
        Baseline \passattop{10} &\coloryellow $46.6$ &\coloryellow $12.8$ &\coloryellow $4.9$ \\
        Baseline \passattop{50} & $59.4$ & $23.0$ & $12.1$ \\
        \midrule
        \ours \passattop{1} & \colorblue $34.6$~\improve{7.4} & \colorblue $8.1$~\improve{2.9} & \colorblue $2.2$~\improve{0.4} \\
        \ours \passattop{2} & $41.2$ & $11.2$ & $4.1$ \\
        \ours \passattop{10} &\coloryellow $53.2$~\improve{6.6} &\coloryellow $18.1$~\improve{5.2} &\coloryellow $8.6$~\improve{3.7} \\
        \bottomrule
        \end{tabular}
    }
    \caption{Pass@$k$ ($\%$) results on the APPS benchmark (zero-shot) using \davincitwo with respect to different levels of difficulty.}
    \label{tab:apps_zeroshot}
\end{table}

\begin{table}[t]
    \centering
    \scalebox{1}{
        \begin{tabular}{ccccccc}
        \toprule
        \multicolumn{4}{c}{{\textbf{Baseline}}} & \multicolumn{3}{c}{{\textbf{\ours}}} \\
        \cmidrule(lr){1-4}
        \cmidrule(lr){5-7}
        \multicolumn{1}{c}{Pass@$1$} &\multicolumn{1}{c}{Pass@$10$} & \multicolumn{1}{c}{Pass@$100$}& \multicolumn{1}{c}{Pass@$1000$} & \multicolumn{1}{c}{Pass@$1$} & \multicolumn{1}{c}{Pass@$10$} & \multicolumn{1}{c}{Pass@$100$} \\
        \midrule
        \colorblue $0.7$ & \coloryellow $3.0$ & \colorgreen $7.5$ & $13.9$ & \colorblue $2.1$~\improve{1.4} & \coloryellow $5.3$~\improve{2.3} & \colorgreen $9.9$~\improve{2.4} \\
        \bottomrule
        \end{tabular}
    }
    \caption{Pass@$k$ ($\%$) results on the CodeContests benchmark (zero-shot) using \davincitwo.}
    \label{tab:codecontests_zeroshot}
\end{table}
\fi




\subsection{Analysis on Test Cases}
\label{sec:exp_test}
The test cases are vital to \ours since the core idea is based on test-driven execution agreement. Hence, in this subsection, we analyze the test cases by answering the following research questions.

%we would like to evaluate the quality of generated test cases, and also explore whether better test cases can further boost the performance of mediocre models.

%It naturally elicits two research questions: 1. What is the actual quality of generated test cases? 2. Will it improve the performance of a mediocre model by equipping better test cases? 

\textbf{Q1. What is the quality of the generated test cases?}
\label{sec:toxic_test_cases}

\begin{figure*}[t]
	\centering
	\begin{subfigure}[t]{0.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{test_case_acc.pdf}
		\caption{}
		\label{subfig:test_case_acc}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{test_case_toxic.pdf}
		\caption{}
		\label{subfig:test_case_toxicity}
	\end{subfigure}
	\caption{The distributions of (a) test case accuracy and (b) toxicity rate for each problem on HumanEval. Test cases are of better quality if they have higher accuracy and lower toxicity rate.}
	\label{fig:test_case_acc_toxicity}
\end{figure*}

%When generating test cases for the HumanEval benchmark, we sample $100$ times for each problem and extract the first five syntactically correct test cases from each sample, which means each problem is equipped with $500$ test cases at most. 
%The actual numbers of extracted test cases 
%for each problem with different models 
%are summarized in Appendix \ref{appendix_stat_test}. 
%To investigate the quality of test cases, we first evaluate their correctness using the canonical solutions provided by the HumanEval benchmark. 
We evaluate the correctness of the generated test cases using the canonical solutions.  
A test case is considered correct if the canonical solution can pass it. Figure \ref{subfig:test_case_acc} summarizes the distributions of test case accuracy on HumanEval, where the horizontal axis represents the accuracy value for each problem and the vertical axis represents the probability density of problems with the corresponding accuracy value. We can see that the test cases generated by Codex models are of much higher accuracy than \codegen/\incoder.
Besides accuracy, we also introduce the test case toxicity rate as a measurement of quality. We consider a test case to be ``toxic" if any generated code solution can pass it while the canonical solution cannot. 
%We consider a test case `toxic' if it has positive execution result with any generated code solution but has negative result with the canonical solution. 
Toxic test cases may hinder the scoring of consensus sets and lead to the failure of \ours. As shown in Figure \ref{subfig:test_case_toxicity}, we can find that the toxicity rate highly correlates to the test case accuracy with respect to different models, where the proportions of toxic test cases for Codex models are smaller than \codegen/\incoder. 
We also evaluate the code coverage of generated test cases using two coverage criterias in Appendix \ref{appendix_coverage}, where Codex models still outperform \codegen/\incoder with an average coverage of over $95\%$.
%\fj{Besides accuracy and toxicity, we also evaluate the code coverage of generated test cases using two coverage criterias. Results are shown in Appendix \ref{appendix_coverage}, where Codex models still outperforms \codegen/\incoder, reaching an average of over $95\%$ coverage.} 
Comparing the test case quality and the performance of \ours shown in Table \ref{tab:main}, we can find that the quality of test cases strongly correlates to the performance gain using \ours concerning different models. 

%For test case generation, we sample 100 times for each problem and extract the first 5 syntactical test cases of each sample, which means each problem is equipped with up to 500 generated test cases. Table \ref{tab:test_case_number} summarizes the average and median number of the extracted test cases for each problem. According to the numbers, all the models except \codegen could generate considerable syntactical test cases. We find plenty of unexpected noise after carefully inspecting the generated content of \codegen, which may be due to the mismatch between \codegen and our prompt design for test case generation. Considering the good performance \codegen achieves through \ours and to keep consistent with the other models, we make no additional modifications to the prompt format for \codegen.

%Figure \ref{subfig:test_case_acc} summarizes the distribution of test case accuracy, where the horizontal axis denotes the test case accuracy value for each problem and the vertical axis denotes the probability density of problems having the corresponding accuracy value.
% We can find that half of the problems have less than 40\% correct test cases using \incoder, \codegen, \cushman and \davincione. While the quality of test cases generated by \davincitwo is much better than the others, which facilitates \davincitwo gaining greater improvement through \ours. 

% \paragraph{Test Case Toxicity}
% There is chance that a generated test case has positive execution results with several generated code solutions, but cannot pass the canonical solution. Such test cases may hinder the execution agreement of \ours and we denote them as \textit{toxic} ones. To estimate the influence of this issue, we investigate the  distribution of test case toxicity rate on the HumanEval benchmark and show the statistics in Figure \ref{subfig:test_case_toxicity}. Specifically, we utilize the execution results when calculating test case accuracy and performing execution agreement to localize the test cases that cannot pass the canonical solution but are able to pass any generated solution. Then we get the test case toxicity rate for each problem by using the number of extracted test cases to divide the number of toxic ones. 

% According to the toxicity rate distribution summarized in Figure \ref{subfig:test_case_toxicity}, toxic test cases occupy a considerable proportion, especially for \incoder, leading to the minor performance improvement through \ours.
% From the results shown in Figure \ref{fig:test_case_acc_toxicity},  we can find the toxicity rate highly related to the original accuracy of test cases with respect to different models. It explains why \incoder has minor performance improvement on the HumanEval benchmark through \ours in contrast to \davincitwo.

\begin{table}[t]
    \centering
    \scalebox{0.9}{
        \begin{tabular}{lllllll}
        \toprule
         \multicolumn{1}{c}{{\textbf{Benchmarks}}} & \multicolumn{3}{c}{{\textbf{HumanEval}}} & \multicolumn{3}{c}{{\textbf{MBPP}}} \\
        \cmidrule(lr){1-1}
        \cmidrule(lr){2-4}
        \cmidrule(lr){5-7}
        \multicolumn{1}{c}{$k$}& \multicolumn{1}{c}{$1$} &\multicolumn{1}{c}{$2$} & \multicolumn{1}{c}{$10$}& \multicolumn{1}{c}{$1$} & \multicolumn{1}{c}{$2$} & \multicolumn{1}{c}{$10$} \\
        \midrule
        \cushman & $47.1$~\improveorange{2.6} & $58.6$~\improveorange{8.5} & $71.2$~\improveorange{5.5} & $59.7$~\improveorange{4.3} & $64.8$~\improveorange{3.1} & $75.5$~\improveorange{2.8} \\
        \davincione & $52.0$~\improveorange{1.8} & $62.9$~\improveorange{4.0} & $78.1$~\improveorange{2.3} & $64.3$~\improveorange{2.4} & $71.7$~\improveorange{2.6} & $80.5$~\improveorange{1.2}  \\
        \incoderb & $26.8$~\improveorange{6.2} & $30.4$~\improveorange{2.8} & $40.8$~\improveorange{3.7} & $50.3$~\improveorange{15.9} & $55.4$~\improveorange{11.5} & $64.5$~\improveorange{6.3} \\
        \codegenb & $47.7$~\improveorange{11.0} & $54.9$~\improveorange{10.2} & $71.0$~\improveorange{11.7} & $60.0$~\improveorange{10.5} & $67.6$~\improveorange{11.0} & $76.5$~\improveorange{8.0}  \\
        \bottomrule
        \end{tabular}
    }
    \caption{Pass@$k$ ($\%$) on the HumanEval and MBPP benchmarks with \cushman, \davincione, \incoder, and \codegen using the test cases generated by \davincitwo. The numbers in {\textcolor{orange}{orange}} indicate the absolute improvements of \passattop{k} using \davincitwo test cases over that using their own generated test cases.
    }
    \label{incoder&codegen&davinci}
\end{table}

%\paragraph{Using stronger model to generate test case for weaker model}
\textbf{Q2. Can better test cases further boost the performance of mediocre models?}

From the above discussion with Figure \ref{fig:test_case_acc_toxicity}, we can find that \davincitwo is the most capable model for generating high-quality test cases. 
Hence, we conduct an experiment to boost the performance of the other four models (\cushman, \davincione, \incoder, and \codegen) using test cases generated by \davincitwo. 
%Hence, we conduct an experiment to demonstrate the effectiveness of performing execution agreement using test cases generated by \davincitwo and code solutions generated by the other four models (\cushman, \davincione, \incoder, and \codegen). 
Table \ref{incoder&codegen&davinci} summarizes the performance gain with respect to different models on the HumanEval and MBPP benchmarks. In general, using the test cases generated by \davincitwo can significantly improve the performance of using the test cases generated by the less capable models themselves. For \cushman and \davincione, the absolute improvements are in the range of $1.8\%$ to $4.3\%$ on \passattop{1}, while for \incoder and \codegen, the range is from $6.2\%$ to $15.9\%$. 
The above results indicate that the correct code solutions generated by mediocre models can be further exploited by adopting better test cases.

\textbf{Q3. How effective is \ours when there are fewer test cases?}

\begin{wraptable}{l}{5.2cm}
        \centering
        \scalebox{0.85}{
            \begin{tabular}{cllll}
            \toprule
            \multirow{3}{*}{\textbf{\textit{Limit}}} & \multicolumn{4}{c}{\textbf{Sampling Number}} \\
            \cmidrule(lr){2-5}
            & $10$ & $20$ & $50$ & $100$ \\
            \midrule
            $1$ & $56.5$ & $57.5$ & $60.7$ & $62.4$ \\
            $2$ & $62.2$ & $62.8$ & $63.2$ & $63.6$ \\
            $3$ & $62.9$ & $63.2$ & $65.5$ & $65.0$ \\
            $4$ & $64.1$ & $64.5$ & $65.7$ & $65.0$ \\
            $5$ & $63.9$ & $64.2$ & $65.2$ & $65.8$ \\
            \bottomrule
            \end{tabular}
        }
        \caption{Pass@$1$ ($\%$) on HumanEval using \ours and \davincitwo with different numbers of test cases. \emph{Sampling Number} denotes the number of samples generated by model, and \emph{Limit} denotes the test cases extracted per sample.}
        \label{table:fewertest}
\end{wraptable} 

When generating test cases for the HumanEval benchmark, we sample $100$ times for each problem and each sample may include multiple assertion statements (i.e., test cases), denoted as \emph{Sampling Number} $=100$. Then we extract the first $5$ syntactically correct test cases from each sample, denoted as \emph{Limit} $=5$. This means each problem is equipped with $500$ test cases at most. 
The actual numbers of extracted test cases are summarized in Appendix \ref{appendix_stat_test}. We perform an ablation study on the number of test cases by decreasing \emph{Sampling Number} and \emph{Limit}. As shown in Table \ref{table:fewertest}, we can conclude that using more test cases in \ours could generally lead to better performance, while the performance gap narrows when \emph{Sampling Number} $\geq 50$ and \emph{Limit} $\geq 3$. Moreover, \ours improves the pass@$1$ by $9.5\%$ with only $10$ test cases using \davincitwo, suggesting the high test case efficiency. We can use a smaller \emph{Sampling Number} in real-world application to balance the performance and computation cost. More results can be found in Appendix \ref{appendix_test_case_number}.

%Furthermore, we are interested in another question: how effective is \ours when there are fewer test cases? In Appendix \ref{appendix_test_case_number}, we perform an ablation study on reducing the number of test cases used by \ours on the HumanEval benchmark. The results suggest that \ours has high test case efficiency, improving the pass@$1$ by $9.5\%$ with only $10$ test cases using \davincitwo.

%\fj{Furthermore, we notice that a considerable amount of test cases (up to $500$ per problem) are sampled for \ours. So here is the third research question we hope to answer, how effective is \ours when there are less available test cases? In Appendix \ref{appendix_test_case_number}, we perform an ablation study on reducing the number of test cases used by \ours for the HumanEval benchmark. Results show that \ours has high test case efficiency, where it can improve the baseline \passattop{1} performance by absolute $9.5\%$ using \davincitwo with only $20$ test cases.}


\subsection{Case Study}
\label{sec:case_study}

\iffalse
\begin{minipage}{.515\textwidth}
\begin{lstlisting}[style=mypython, label={lst:good_example}, basicstyle=\tiny]
def below_threshold(l: list, t: int):
    """
    Return True if all numbers in the list l are below
    threshold t.
    """
    # ground truth test cases
    # ([1, 2, 4, 10], 100) => True
    # ([1, 8, 4, 10], 10) => False
    
    # below is an example from the consensus
    # set that contains 61 correct solutions
    # and 218 test cases
    if l == []:
        return True
    return l[0] < t and below_threshold(l[1:], t)
    
    # below is an example from the consensus set that
    # contains 30 incorrect solutions 
    # and 226 test cases
    for e in l:
        if e > t:
            return False
    return True
\end{lstlisting}
\end{minipage}
\hspace{0.1cm}
\begin{minipage}{.45\textwidth}
\begin{lstlisting}[style=mypython, label={lst:bad_example}, basicstyle=\tiny]
def minSubArraySum(nums):
    """
    Given an array of integers nums, find the 
    minimum sum of any non-empty sub-array
    of nums.
    """
    # ground truth test cases
    # [100, -33, 32, -1, 0, -2] => -33
    # [-1, -2, -3, 10, -5] => -6
    
    # an example from the largest consensus set
    # that contains the incorrect solutions
    if not nums:
        return 0
    total = nums[0]
    min_sum = total
    for i in range(1, len(nums)):
        if total < 0:
            total = nums[i]
        else:
            total += nums[i]
        min_sum = min(min_sum, total)
    return min_sum
\end{lstlisting}
\end{minipage}
\fi

\begin{figure*}[t]
	\centering
	\begin{subfigure}[t]{0.395\linewidth}
		\centering
		\includegraphics[width=\linewidth]{case-main1-1.pdf}
		\caption{}
		\label{subfig:case_main1}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.59\linewidth}
		\centering
		\includegraphics[width=\linewidth]{case-main3-1.pdf}
		\caption{}
		\label{subfig:case_main2}
	\end{subfigure}
	\caption{Two real cases from the HumanEval benchmark with \ours and \cushman.}
	\label{fig:case_main}
\end{figure*}

In \ours, we design the dual execution agreement based on the idea that a good code solution can pass the most test cases and agree with the most solutions of the same functionality. We use ``dual" because both the code solutions and the test cases are critical. 
Figure \ref{subfig:case_main1} shows a case from the HumanEval benchmark using \cushman. The highest scoring consensus set has the correct functionality that returns true if all numbers in the list are below threshold $t$, while the consensus set ranked $2$ does not understand the boundary condition exactly. The solutions in the second consensus set can pass more test cases (i.e., $226$) than that in the first consensus set (i.e., $218$). However, considering both code solutions and test cases, \ours can successfully rank the consensus sets and find the correct solutions. 
Such cases are not rare, suggesting that our design of the dual execution agreement is reasonable. For further statistical demonstration, we conduct an ablation study to score the consensus set by considering only the number of code solutions or test cases. The results again support our claim, as detailed in Appendix \ref{appendix_simplecount}.

%Moreover, we conduct an ablation study in Appendix \ref{appendix_simplecount} to score the consensus sets by considering only the number of code solutions or test cases, further statistically demonstrating the plausibility of our dual execution agreement.


%According to Figure \ref{fig:agree} and Appendix \ref{appendix_simplecount}, we can conclude that the number of passed test cases does not always correlate to the correctness of code solutions. As for \ours, we rank the solutions based on the functional consensus, which will take into account the importance of both code solutions and test cases. Figure \ref{lst:good_example} is an example demonstrating the effectiveness of \ours, where we have two code solutions generated by \cushman for a problem in the HumanEval benchmark, and the solutions are from the first  and second largest consensus sets respectively. There are 61 correct solutions that can pass a total of 218 test cases. While there are 30 solutions passing more (226) test cases even though they misunderstand the scope of the threshold. In this example, \ours can exactly tell the correct solutions from others. We list some similar examples in Appendix \ref{} for reference.


%Comparing the \ours pass@$1$ with the baseline pass@$100$ in Table \ref{tab:main}, we can see that there is still room for performance improvement. As mentioned in Section \ref{sec:toxic_test_cases}, there are incorrect code solutions that can pass the ``toxic'' test cases, which may hinder the scoring of consensus sets. For \ours with \cushman on the HumanEval benchmark, we find $53$ out of $164$ programming problems where at least one of the generated code solutions is correct, but the top $1$ scoring consensus set is incorrect. We manually investigate the code solutions in the incorrect top $1$ consensus sets, and find that most of them (i.e., code solutions of $43$ problems) should be blamed on the model's misunderstanding of the problem descriptions. Figure \ref{subfig:case_main2} shows a real case that the correct solutions are in the consensus set ranked $3$. Apart from the dominate misunderstanding issue, there are other minor issues, such as ambiguous problem description and uncovered corner cases. Hope this error analysis can provide inspiration for future study. More real cases can be found in Appendix \ref{appendix_code_example}.

\ours is empowered by the pre-trained language models, but is also limited by them. Therefore, the second assumption made in Section \ref{sec:agree} does not always hold, leading to error cases where the correct code solution is generated, but not in the top $1$ consensus set. For \ours with \cushman on the HumanEval benchmark, we find $53$ out of $164$ programming problems that belong to this situation. We manually investigated these problems and found that $20\%$ of them can be blamed on issues such as ambiguous problem descriptions, uncovered corner cases, and lack of import statements, while the remaining problems are attributed to the failure of the model to understand the problem descriptions. Figure \ref{subfig:case_main2} shows an error case caused by ambiguity. The correct understanding of the description ``sum(first index value, last index value)'' is to add the first and last values, while the code solutions that sum all values from the first to the last are ranked top $1$. More real cases can be found in Appendix \ref{appendix_code_example}. And hope the error analysis can provide inspiration for future studies on improving code generation for more difficult programming problems. 


%Comparing the \ours pass@$1$ with the baseline pass@$100$ in Table \ref{tab:main}, we can see that there is still room for performance improvement. As mentioned in Section \ref{sec:toxic_test_cases}, there are incorrect code solutions that can pass the ``toxic'' test cases, which may hinder the scoring of consensus sets. For \ours with \cushman on the HumanEval benchmark, we find $53$ out of $164$ programming problems where at least one of the generated code solutions is correct, but the top $1$ scoring consensus set is incorrect. We manually investigate the code solutions in the incorrect top $1$ consensus sets, and find that most of them (i.e., code solutions of $43$ problems) should be blamed on the model's misunderstanding of the problem descriptions. Figure \ref{subfig:case_main2} shows a real case that the correct solutions are in the consensus set ranked $3$. Apart from the dominate misunderstanding issue, there are other minor issues, such as ambiguous problem description and uncovered corner cases. Hope this error analysis can provide inspiration for future study. More real cases can be found in Appendix \ref{appendix_code_example}.


%Nonetheless, according to the results of \ours in Table \ref{tab:main} and Table \ref{tab:apps_code}, there is still room for performance improvement. As mentioned in Section \ref{sec:toxic_test_cases}, there are incorrect code solutions that can pass the ``toxic'' test cases, which may hinder the scoring of consensus sets. We manually investigate the code solutions generated by \cushman for the HumanEval benchmark where the problems have at least one correct solution while their largest consensus sets contain no correct solutions. Eventually we find $53$ out of $164$ problems in the benchmark pertain to such issue and most ($43$) of them should blame the model's misunderstanding of the problem descriptions. Figure \ref{subfig:case_main2} shows an example that the generated code solutions in the largest consensus set are not solving the given problem while they can pass more generated test cases. Apart from the dominate misunderstanding issue, there are other minor issues (e.g., ambiguous problem description, failing corner cases) that could cause such failure. We also list some examples in Appendix \ref{appendix_code_example} for reference.

% We manually examine the ``toxic'' code solutions generated by \cushman for the HumanEval benchmark and list three representative examples in the following. Code Example \ref{lst:code1} demonstrates that an ambiguous problem description can lead to different reasonable solutions. In this example, the \#1 solution sees the \textit{sum(first index value, last index value)} as the accumulated sum of the array. While the actual meaning of the statement is to add the first and the last numbers of the array. Code Example \ref{lst:code2} demonstrates that the generated solutions may fail at corner cases. In this example, the \#1 solution almost tackles the \textit{even\_odd\_count} problem except that a negative \textit{num} argument will lead to a dead loop. Code Example \ref{lst:code3} demonstrates that the code generation model will not always understand the programming problems. In this example, the \#1 solution is totally missing the point of finding a \textit{sub-array of nums} that has the minimum sum. Unfortunately, since the model has a misunderstanding of the problem, it also generates more test cases to support the \#1 solution instead of the correct \#2 solution. 

% We perform experiments that generate test cases using a better model with the goal of improving performance of weaker ones. The idea is better test cases quality will likely bootstrap the code generation process through \ours test-driven execution mechanism. Table \ref{incoder&codegen&davinci} demonstrates the effectiveness of using \davincitwo model which achieves the best performance across HumanEval and MBPP dataset to generate test cases for \incoder, \codegen, \cushman, and \davincione models. 
% In general, using test cases generated by \davincitwo improves \ours \passattop{1} performance significantly for \incoder and \codegen, with the improvement in the range of $6.2\%\sim15.9\%$. Nevertheless, the improvement is not obvious for \cushman and \davincione. Such results may attribute to the difference in the quality of generated test cases. According to Figure \ref{fig:test_case_acc_toxicity}, \incoder and \codegen have much lower test case accuracy compared to Codex models, thus could further exploit the potential of code solutions through \ours based on better test cases.
% In general, using test cases generated by \davincitwo model improves \ours pass@top-1 results significantly, the improvement are in the range of $6.2\%\sim15.9\%$, with the result of \incoder model on MBPP achieves the best gain of $15.9\%$ improvement.



%\paragraph{Edited Benchmark}
%\paragraph{Hyper Parameter Tuning}

%\paragraph{Case Study}
% We find some code solutions are able to pass all the ground truth test cases as well as the \textit{toxic} test cases, which should not happen in theory. There are two reasons that could cause such issue. One is the wrong canonical solutions, for example, the canonical solution for a programming problem in HumanEval overlooks the case when input list is empty. The other reason is the biased ground truth test cases, for example, the ground truth test cases for a problem in HumanEval overlap the situation when input string contains characters other than parentheses.

% toxic test case study; no valid test case




==> CodeT_ Code Generation with Generated Tests (arXiv V2 20221123)/5_related_work.tex <==
\section{Related Work}

%\paragraph{Code Generation with Large Models} Recently, a number of large pre-trained language models have been proposed for code generation. Benefiting from billions of trainable parameters and massive publicly available source code, models could achieve surprisingly good performance. For instance, AlphaCode~\citep{li2022competition} claimed to have outperformed half of the human competitors in real-world programming competitions, and Codex~\citep{chen2021evaluating} is empowering  \href{https://github.com/features/copilot/}{Copilot} to provide real-time coding suggestions. In addition to the private-access AlphaCode and Codex models, there are also open-source code generation models like GPT-Neo~\citep{gpt-neo}, GPT-J~\citep{gpt-j}, CodeParrot~\citep{tunstall2022natural}, PolyCoder~\citep{xu2022PolyCoder}, \codegen~\citep{Nijkamp2022ACP}, and \incoder~\citep{dfried2022incoder}. In our study, we take advantage of the Codex inference API provided by OpenAI as well as the two competitive open-source models \codegen and \incoder to perform zero-shot code generation.

\paragraph{Code Generation with Large Models} Recently, a number of large pre-trained language models have been proposed for code generation. Benefiting from billions of trainable parameters and massive publicly available source code, models could achieve surprisingly good performance. For instance, AlphaCode~\citep{li2022competition} claimed to have outperformed half of the human competitors in real-world programming competitions, and Codex~\citep{chen2021evaluating} is empowering  \href{https://github.com/features/copilot/}{Copilot} to provide real-time coding suggestions. Other open-source code generation models include GPT-Neo~\citep{gpt-neo}, GPT-J~\citep{gpt-j}, CodeParrot~\citep{tunstall2022natural}, PolyCoder~\citep{xu2022PolyCoder}, \codegen~\citep{Nijkamp2022ACP}, and \incoder~\citep{dfried2022incoder}. In our study, we take advantage of the Codex inference API provided by OpenAI as well as the two competitive open-source models \codegen and \incoder to perform zero-shot code generation.

\paragraph{Automatic Test Case Generation} Automated test case generation for programming problems can reduce the effort of writing test cases manually by developers. Early works including Randoop~\citep{randoop}, EvoSuite~\citep{evosuite}, MOSA~\citep{mosa},  DynaMOSA~\citep{dynamosa}, and MIO~\citep{mio}, were proposed to automatically generate test cases for statically typed programming languages like Java. The later proposed Pynguin~\citep{pynguin} could handle dynamically typed language like Python. Nevertheless, they are all search-based heuristics methods, which have limitations to the diversity and quantity of generated test cases. To combat these limitations, recently proposed approaches~\citep{AthenaTest,li2022competition} leveraged pre-trained language models like BART~\citep{bart} and T5~\citep{t5} fine-tuned on labelled data for test case generation. Unlike previous works that require heuristic rules or model training, we directly sample test cases from powerful code generation models like Codex in the zero-shot setting with elaborate prompts.

\paragraph{Code Selection from Multiple Samples} Despite large models have achieved great performance in code generation, the models need to sample many times to find the correct answer. %, which brings the challenge to select the correct ones from multiple samples. 
Recently, several approaches were proposed to tackle this issue. 
In the domain of solving math word problems, \cite{cobbe2021training} chose the one with highest rank by a trained verifier, and \cite{shen2021generate} proposed to jointly train the generator and ranker through a multi-task framework. In the domain of general purpose code generation, \cite{inala2022fault} trained a fault-aware ranker. Moreover, some work has been proposed to leverage the execution information \citep{shi2022natural,li2022competition,le2022coderl,lahiri2022interactive}. %Apart from execution information, \cite{lahiri2022interactive} also leveraged the interaction with humans to select the correct code solutions. % by ranking the similarity of outputs based on the given inputs. 
%As for the input data, \cite{shi2022natural} employed the test cases provided by the benchmark, while \cite{li2022competition} trained an additional generator. 
%\cite{wang2022self} propose to improve the reasoning performance of large models by sampling a number of diverse reasoning paths and then choose the most consistent answer. \cite{li2022advance} proposed to verify the correctness of each single reasoning step by a voting verifier.
Unlike previous works that require model training or pre-existing test cases or user interactions, we let the large models generate test cases for themselves and automatically rank the solutions based on the test-driven dual execution agreement. 
The idea of ranking based on agreement also appears in the domain of reasoning \citep{wang2022self,li2022advance}. %\cite{lahiri2022interactive} also tried to exploit the tests generated from large models to improve the quality of code generation. Their objective is to utilize user interactions to provide guarantees on the suggested code. While our approach is to automatically rank the solutions based on their test-driven dual execution agreement.



==> CodeT_ Code Generation with Generated Tests (arXiv V2 20221123)/6_conclusion.tex <==
\section{Conclusion and Future Work}
In this paper, we propose a simple yet effective approach, called \ours, leveraging pre-trained language models to generate both the code solutions and the test cases. \ours executes the code solutions using the test cases and chooses the best solution based on the dual execution agreement. We demonstrate the dual agreement with both the test cases and other solutions is critical to the success of \ours, perform a thorough analysis on the quality of generated test cases and their impact on \ours, and study cases to provide more insights. Experimental results clearly demonstrate the superiority of \ours, improving the pass@$1$ numbers significantly on various benchmarks. 
While there remain challenges that \ours only works for executable code generation and it introduces extra computation cost for test case generation. 
In future work, we will explore the ways to tackle these challenges and improve \ours to solve more difficult programming problems. 

%Furthermore, the combination of \davincitwo and \ours surprisingly improves the pass@$1$ on HumanEval to  $65.8\%$, an absolute $20$+$\%$ improvement over the previous state-of-the-art results. 
%In future work, we are interested in improving \ours to solve more difficult programming problems and extending it to other code-related tasks.
%In future work, we will explore how to combine the ideas of \ours with training a ranker.   Another direction is to extend \ours to other code-related tasks.

%\section*{Acknowledgement}
%We would like to thank Davis Mueller and Jade Huang for proofreading the paper and providing insightful comments.

%Though \ours achieves exceptional performance, there remains challenges to apply it in real-world applications. First, \ours is limited to the tasks that generate executable code, and it may cause unexpected vulnerabilities by executing the generated code directly.

%\fj{Our experiments have proved the effectiveness of \ours, while there remains challenges to employ our approach in real-world application. First, \ours is limited to the tasks that generate executable code, and it may cause unexpected vulnerabilities by executing the generated code directly. Second, \ours will introduce extra computation cost to code generation. Though we have proved the high test case efficiency of \ours, the cost of sampling, execution, and ranking is still indispensable. In the future work, we will also explore the ways to tackle these challenges. For example, using a neural network to mimic the execution process, and evaluating the functional correctness/consensus without test cases.}
